SIGMA: A Structural Inconsistency Reducing Graph Matching Algorithm

Graph matching finds the correspondence of nodes across two correlated graphs and lies at the core of many applications. When graph side information is not available, the node correspondence is estimated on the sole basis of network topologies. In this paper, we propose a novel criterion to measure the graph matching accuracy, structural inconsistency (SI), which is defined based on the network topological structure. Specifically, SI incorporates the heat diffusion wavelet to accommodate the multi-hop structure of the graphs. Based on SI, we propose a Structural Inconsistency reducing Graph Matching Algorithm (SIGMA), which improves the alignment scores of node pairs that have low SI values in each iteration. Under suitable assumptions, SIGMA can reduce SI values of true counterparts. Furthermore, we demonstrate that SIGMA can be derived by using a mirror descent method to solve the Gromov-Wasserstein distance with a novel K-hop-structure-based matching costs. Extensive experiments show that our method outperforms state-of-the-art methods.

==> local_topology arxiv/lib/consistency.tex <==
\newcommand{\RWR}{\text{RWR}}
\newcommand{\MLP}{\text{MLP}}
\newcommand{\MLPh}{\text{MLP-}} % here h means hyphen
\newcommand{\LSTM}{\text{LSTM}}
\newcommand{\LSTMh}{\text{LSTM-}}
\newcommand{\leakyrelu}{\text{LeakyReLU}}
\newcommand{\recall}{\text{recall}}
\newcommand{\precision}{\text{precision}}
\newcommand{\Fone}{\text{F1}}
\newcommand{\name}{\text{PGM}}
\newcommand{\nameh}{\text{PGM}}

\newcommand{\dataset}{dataset}
\newcommand{\datasets}{datasets}
\newcommand{\groundtruth}{ground truth}
\newcommand{\hyperparameter}{hyperparameter}
\newcommand{\kmeans}{$k$-means}
\newcommand{\minibatch}{mini-batch}
\newcommand{\nonconvex}{non-convex}
\newcommand{\nonzero}{nonzero}
\newcommand{\realworld}{real-world}
\newcommand{\stepsize}{stepsize}
\newcommand{\suboptimal}{sub-optimal}
\newcommand{\subproblem}{sub-problem}
\newcommand{\subproblems}{sub-problems}


\newcommand{\Dataset}{Dataset}
\newcommand{\Datasets}{Datasets}
\newcommand{\Groundtruth}{Ground truth}
\newcommand{\Minibatch}{Mini-batch}
\newcommand{\Nonconvex}{Non-convex}
\newcommand{\Realworld}{Real-world}

==> local_topology arxiv/lib/symbol.tex <==
\newcommand{\AB}{\mathbf{A}}
\newcommand{\BB}{\mathbf{B}}
\newcommand{\CB}{\mathbf{C}}
\newcommand{\DB}{\mathbf{D}}
\newcommand{\EB}{\mathbf{E}}
\newcommand{\FB}{\mathbf{F}}
\newcommand{\GB}{\mathbf{G}}
\newcommand{\HB}{\mathbf{H}}
\newcommand{\IB}{\mathbf{I}}
\newcommand{\JB}{\mathbf{J}}
\newcommand{\KB}{\mathbf{K}}
\newcommand{\LB}{\mathbf{L}}
\newcommand{\MB}{\mathbf{M}}
\newcommand{\NB}{\mathbf{N}}
\newcommand{\OB}{\mathbf{O}}
\newcommand{\PB}{\mathbf{P}}
\newcommand{\QB}{\mathbf{Q}}
\newcommand{\RB}{\mathbf{R}}
\newcommand{\SB}{\mathbf{S}}
\newcommand{\TB}{\mathbf{T}}
\newcommand{\UB}{\mathbf{U}}
\newcommand{\VB}{\mathbf{V}}
\newcommand{\WB}{\mathbf{W}}
\newcommand{\XB}{\mathbf{X}}
\newcommand{\YB}{\mathbf{Y}}
\newcommand{\ZB}{\mathbf{Z}}
\newcommand{\OmegaB}{\mathbf{\Omega}}
\newcommand{\zeroB}{\mathbf{0}}
\newcommand{\oneB}{\mathbf{1}}
\newcommand{\aB}{\mathbf{a}}
\newcommand{\bB}{\mathbf{b}}
\newcommand{\cB}{\mathbf{c}}
\newcommand{\dB}{\mathbf{d}}
\newcommand{\eB}{\mathbf{e}}
\newcommand{\fB}{\mathbf{f}}
\newcommand{\gB}{\mathbf{g}}
\newcommand{\hB}{\mathbf{h}}
\newcommand{\iB}{\mathbf{i}}
\newcommand{\jB}{\mathbf{j}}
\newcommand{\kB}{\mathbf{k}}
\newcommand{\lB}{\mathbf{l}}
\newcommand{\mB}{\mathbf{m}}
\newcommand{\nB}{\mathbf{n}}
\newcommand{\oB}{\mathbf{o}}
\newcommand{\pB}{\mathbf{p}}
\newcommand{\qB}{\mathbf{q}}
\newcommand{\rB}{\mathbf{r}}
\newcommand{\sB}{\mathbf{s}}
\newcommand{\tB}{\mathbf{t}}
\newcommand{\uB}{\mathbf{u}}
\newcommand{\vB}{\mathbf{v}}
\newcommand{\wB}{\mathbf{w}}
\newcommand{\xB}{\mathbf{x}}
\newcommand{\yB}{\mathbf{y}}
\newcommand{\zB}{\mathbf{z}}
\newcommand{\ABB}{\mathbb{A}}
\newcommand{\NBB}{\mathbb{N}}
\newcommand{\PBB}{\mathbb{P}}
\newcommand{\RBB}{\mathbb{R}}
\newcommand{\SBB}{\mathbb{S}}
\newcommand{\XBB}{\mathbb{X}}
\newcommand{\YBB}{\mathbb{Y}}
\newcommand{\VBB}{\mathbb{V}}
\newcommand{\EBB}{\mathbb{E}}
\newcommand{\AM}{\mathcal{A}}
\newcommand{\BM}{\mathcal{B}}
\newcommand{\CM}{\mathcal{C}}
\newcommand{\EM}{\mathcal{E}}
\newcommand{\FM}{\mathcal{F}}
\newcommand{\GM}{\mathcal{G}}
\newcommand{\HM}{\mathcal{H}}
\newcommand{\IM}{\mathcal{I}}
\newcommand{\LM}{\mathcal{L}}
\newcommand{\MM}{\mathcal{M}}
\newcommand{\NM}{\mathcal{N}}
\newcommand{\OM}{\mathcal{O}}
\newcommand{\PM}{\mathcal{P}}
\newcommand{\SM}{\mathcal{S}}
\newcommand{\TM}{\mathcal{T}}
\newcommand{\UM}{\mathcal{U}}
\newcommand{\VM}{\mathcal{V}}
\newcommand{\WM}{\mathcal{W}}
\newcommand{\XM}{\mathcal{X}}
\newcommand{\YM}{\mathcal{Y}}
\newcommand{\xT}{\tilde{\mathbf{x}}}
\newcommand{\yT}{\tilde{\mathbf{y}}}
\newcommand{\zT}{\tilde{\mathbf{z}}}
\newcommand{\dHat}{\hat{\mathbf{d}}}
\newcommand{\DHat}{\hat{\mathbf{D}}}
\newcommand{\xHat}{\hat{\mathbf{x}}}
\newcommand{\alphaB}{\mbox{\boldmath$\alpha$\unboldmath}}
\newcommand{\betaB}{\mbox{\boldmath$\beta$\unboldmath}}
\newcommand{\gammaB}{\mbox{\boldmath$\gamma$\unboldmath}}
\newcommand{\etaB}{\mbox{\boldmath$\eta$\unboldmath}}
\newcommand{\epsilonB}{\mbox{\boldmath$\epsilon$\unboldmath}}
\newcommand{\phiB}{\mbox{\boldmath$\phi$\unboldmath}}
\newcommand{\piB}{\mbox{\boldmath$\pi$\unboldmath}}
\newcommand{\PhiB}{\mbox{\boldmath$\Phi$\unboldmath}}
\newcommand{\PsiB}{\mbox{\boldmath$\Psi$\unboldmath}}
\newcommand{\thetaB}{\mbox{\boldmath$\theta$\unboldmath}}
\newcommand{\ThetaB}{\mbox{\boldmath$\Theta$\unboldmath}}
\newcommand{\muB}{\mbox{\boldmath$\mu$\unboldmath}}
\newcommand{\nuB}{\mbox{\boldmath$\nu$\unboldmath}}
\newcommand{\sigmaB}{\mbox{\boldmath$\sigma$\unboldmath}}
\newcommand{\SigmaB}{\mbox{\boldmath$\Sigma$\unboldmath}}
\newcommand{\xiB}{\mbox{\boldmath$\xi$\unboldmath}}
\newcommand{\XiB}{\mbox{\boldmath$\Xi$\unboldmath}}
\newcommand{\zetaB}{\mbox{\boldmath$\zeta$\unboldmath}}
\newcommand{\GammaB}{\mbox{\boldmath$\Gamma$\unboldmath}}
\newcommand{\LambdaB}{\mbox{\boldmath$\Lambda$\unboldmath}}
\newcommand{\lambdaB}{\mbox{\boldmath$\lambda$\unboldmath}}
\newcommand{\omegaB}{\mbox{\boldmath$\omega$\unboldmath}}
\newcommand{\DeltaB}{\mbox{\boldmath$\Delta$\unboldmath}}
\newcommand{\varepsilonB}{\mbox{\boldmath$\varepsilon$\unboldmath}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\rank}{\mathop{\rm rank}}
\newcommand{\sgn}{\mathrm{sgn}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\rk}{\mathrm{rank}}
\newcommand{\diag}{\mathsf{diag}}
\newcommand{\dg}{\mathsf{dg}}
\newcommand{\vect}{\mathsf{vec}}
\newcommand{\etal}{{\em et al.\/}\,}
\newcommand{\ie}{{\em i.e.\/}\,}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand{\prox}{\mathrm{prox}}
\newcommand{\Time}{{\mathbf{Time}}}
\newcommand{\defi}{\stackrel{\mathrm{def}}{=}}
\newcommand{\lk}{{l_k}}
\newcommand{\ik}{{i_k}}
\newcommand{\trace}{\operatorname{trace}}
\newcommand{\proj}{\operatorname{Proj}}
\newcommand{\KL}{\operatorname{KL}}
\newcommand{\Diag}{\operatorname{Diag}}

==> local_topology arxiv/sections/add_experiment.tex <==
\subsection{Additional Experiment Details}\label{sec:additional experimental setup}

We first include more experimental details about parameter choice in this subsection.
For experiments in the main paper, we set the propagation time $t=1\times 10^{-3}$ and the number of hops $K=3$.
%The propagation time $t$ and the number of hops $K$ in Sec. \ref{sec:experiment} are chosen as $1\times 10^{-3}$ and $3$, respectively.
%All codes are implemented in Python 3.6 and the package dependencies are listed in the requirements.txt file in the code submission.
%The experiments are conducted on a Ubuntu server with two CPUs (Intel Xeon (R) CPU E5-2680 v4 @ 2.40GHz), 4 Nvidia 2080 Ti graphics cards, and 378 GB of RAM.

%\subsection{Matching Permutated Networks}

\paragraph{The influence of $K$.}

We empirically study the influence of $K$.
On the one hand, increasing $K$ can increase the distinguishability of nodes and thus boost the matching accuracy.
On the other hand, \method{} with a larger $K$ is easier to be affected by structural noise, as is implied by the upper bound in Theorem \ref{thm:principle}.
Figure \ref{fig:n_hop} demonstrates that $K=3$ can achieve a balance.
With the amount of noise increasing, \method{} with a larger $K$ deteriorates faster.
\method{} with $K=1$ outperforms RefiNA, which demonstrates that \method{} is more related to MNC theoretically.

\begin{figure}[ht]
	\centering
	\includegraphics[width=\textwidth]{imgs/n_hop.pdf}
	\caption{NC of \method{} for different $K$ and $q$. The propagation time $t$ is set as $1\times 10^{-3}$.}\label{fig:n_hop}
\end{figure}

\paragraph{Sensitivity to propagation time $t$.}

The range of propagation time is determined by line search, which is demonstrated in Figure \ref{fig:prop_time}.
On all \datasets{},
\method{} is not sensitive to the choice of propagation time $t$ and achieves good performance when $1\times 10^{-6}\le t\le 1\times 10^{-3}$.
Note that when $t$ is too small, $\PsiB\simeq\IB-t\LB$ where $\IB$ is the identity matrix and \method{} is reduced to only considering one-hop information.
Therefore, the accuracy slightly drops when $t\le 1\times 10^{-5}$.
\begin{figure}[ht]
	\centering
	\includegraphics[width=\textwidth]{imgs/prop_time.pdf}
	\caption{NC of \method{} with varying values of propagation time $t$ when $q=0.25$ for $K=2,3,4$.}\label{fig:prop_time}
\end{figure}





%\paragraph{Mirror descent vs.  gradient descent.}
%Compared to gradient descent-based update,
%the mirror descent based update is more efficient by orders of magnitude,
%as is shown in Figure \ref{fig:md_gd}.
%One can also see from Figure \ref{fig:md_gd} that NC (top row) correlates with the objective value (bottom row) well.
%
%\begin{figure}[ht]
%	\centering
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{imgs/md_gd_nc_yeast.pdf}
%		\caption{PPI Yeast}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{imgs/place.png}
%		\caption{LastFM ASIA}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{imgs/md_gd_nc_arxiv.pdf}
%		\caption{Arxiv}
%	\end{subfigure}
%	\\
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{imgs/md_gd_loss_yeast.pdf}
%		\caption{PPI Yeast}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{imgs/place.png}
%		\caption{LastFM ASIA}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{imgs/md_gd_loss_arxiv.pdf}
%		\caption{Arxiv}
%	\end{subfigure}
%	\caption{Mirror descent vs. gradient descent.}\label{fig:md_gd}
%\end{figure}



%\paragraph{Number of hops.}
%Increasing the number of hops can increase the matching accuracy, as is shown in Figure \ref{fig:n_hop}.
%Setting $K=3$ often yields satisfactory performance.
%
%\begin{figure}[ht]
%	\centering
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{imgs/n_hop_yeast.pdf}
%		\caption{PPI Yeast}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{imgs/place.png}
%		\caption{LastFM ASIA}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{imgs/n_hop_arxiv.pdf}
%		\caption{Arxiv}
%	\end{subfigure}
%	\caption{NC of \method{} with varying $K$.}\label{fig:n_hop}
%\end{figure}
%
\subsection{Matching \Realworld{} Related networks}
%
%\subsubsection{Matching PPI with Real Noise}
%
%We now match the protein-protein network of yeast with high-confidence interactions to its noisy versions that contain $q\%$ more low-confidence interactions where $q\in\{5, 10, 15, 20, 25\}$.
%To better visualize the progress of iterative methods, we report NC v.s. time curves.

%\subsubsection{Matching Time-varying Route-views}

%\begin{table}[ht]
%	\centering
%	\caption{Statistics of Oregon Route Views graphs.}\label{tb:oregon data}
%	\begin{tabular}{lllllll}
%		\toprule
%		\textbf{Dates of RVs} & Mar. 31 & Mar. 31 & Apr. 7 & Apr. 14 &  Apr. 21 & Apr. 28 \\
%		\midrule
%		\textbf{Nodes}  & 10,670        & 10,670        & 10,729       & 10,790       & 10,859       & 10,886       \\
%		\textbf{Edges}  & 22,002        & 22,002        & 21,999       & 22,469       & 22,747       & 22,493      \\
%		\textbf{Diameter (longest shortest path)} & 9 & 9 & 11 & 9 & 10 & 10  \\
%		\bottomrule
%	\end{tabular}
%\end{table}

\begin{table}[ht]
	\centering
	\caption{Statistics of Oregon Route Views graphs.}\label{tb:oregon data}
	\begin{tabular}{c | c | c c c c c}
		\hline
		\multirow{2}{*}{\textbf{Dates of RVs}} & \textbf{Source Graph}  & \multicolumn{5}{|c}{\textbf{Target Graphs}}                                          \\
		& Mar. 31\textsuperscript{st} & Mar. 31\textsuperscript{st} & Apr. 7\textsuperscript{th} & Apr. 14\textsuperscript{th} & Apr. 21\textsuperscript{st} & Apr. 28\textsuperscript{th} \\
		\hline
		\textbf{Nodes}                        & 10,670        & 10,670        & 10,729       & 10,790       & 10,859       & 10,886       \\
		\textbf{Edges}                        & 22,002        & 22,002        & 21,999       & 22,469       & 22,747       & 22,493      \\
		\textbf{Diameters} & 9 & 9 & 11 & 9 & 10 & 10  \\
		\hline
	\end{tabular}
\end{table}

We further demonstrate the performance of \method{} by matching \realworld{} correlated graphs, i.e., the structural difference between the two graphs is induced by \emph{real noise} instead of \emph{simulated noise}.
The experiments are conducted on graphs of Autonomous Systems peering information inferred from Oregon Route-Views (RV) \footnote{\url{http://snap.stanford.edu/data/Oregon-1.html}} between March 31\textsuperscript{st}, 2001 and April 28\textsuperscript{th}, 2001.
The University's RV project\footnote{\url{http://www.routeviews.org/routeviews/}} was a tool for Internet operators to obtain real-time border gateway protocol information about the global routing system.
We match RV on March 31\textsuperscript{st} to RVs between March 31\textsuperscript{st} and April 28\textsuperscript{th}. The \dataset{} statistics are listed in the Table \ref{tb:oregon data}.
We still set $t=1\times 10^{-3}$ and $K=3$ for \method{}.
For fair comparison, RefiNA, MM, GWL, and \method{} use the ouput of CONE-Align to initialize the matching matrix.
%We also study the influence of initializations,
%including the output of CONE-Align \citep{chen2020cone},
%uniform initialization ($T_{ii'}=\frac{1}{|\VM^\tar|}$),
%and random initialization.
% ($T_{i\tilde{i}}=1$ for all $i$ and $\tilde{i}$ is the random)

We report the results on Table \ref{tb:oregon results}.
As RV changes over time, the  performance of all methods decreases except the one on April 28\textsuperscript{th}.
This is possibly due to monthly patterns in RVs.
\method{} outperforms all baselines.
GDD does not take as input the result of CONE-Align and is a deterministic algorithm. The standard deviation is thus 0.
Other 0.000 deviation values are induced by rounding to three decimal places.

\begin{table}[ht]
	\centering
	\caption{NCs on Oregon Route Views graphs across 5 trials.}\label{tb:oregon results}
	\begin{tabular}{c c c c c c}
		\toprule
		$\GM^\tar$ & Mar. 31\textsuperscript{st}     & Apr. 7\textsuperscript{th}      & Apr. 14\textsuperscript{th}     & Apr. 21\textsuperscript{st}     & Apr. 28\textsuperscript{th}      \\
		\midrule
		\textbf{REGAL}         & 0.491 $\pm$ 0.000 & 0.232 $\pm$ 0.001 & 0.189 $\pm$ 0.000 & 0.158 $\pm$ 0.000 & 0.115 $\pm$ 0.000 \\
		\textbf{MM}            & 0.506 $\pm$ 0.004 & 0.314 $\pm$ 0.001 & 0.202 $\pm$ 0.001 & 0.132 $\pm$ 0.000 & 0.173 $\pm$ 0.001  \\
		\textbf{GWL}           & 0.508 $\pm$ 0.002 & 0.362 $\pm$ 0.001 & 0.256 $\pm$ 0.001 & 0.186 $\pm$ 0.000 & 0.229 $\pm$ 0.000  \\
		\textbf{RefiNA}        & 0.259 $\pm$ 0.005 & 0.172 $\pm$ 0.000 & 0.169 $\pm$ 0.000 & 0.110 $\pm$ 0.000 & 0.124 $\pm$ 0.000  \\
		\textbf{GDD}           & 0.341 $\pm$ 0.000 & 0.007 $\pm$ 0.000 & 0.006 $\pm$ 0.000 & 0.007 $\pm$ 0.000 & 0.007 $\pm$ 0.000  \\
		\midrule
		\textbf{\method{}}         & \textbf{0.514 $\pm$ 0.002} & \textbf{0.391 $\pm$ 0.000} & \textbf{0.264 $\pm$ 0.001} & \textbf{0.198 $\pm$ 0.000} & \textbf{0.235 $\pm$ 0.000} \\
		\bottomrule
	\end{tabular}
\end{table}








==> local_topology arxiv/sections/checklist.tex <==
%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%  \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} See Sec. \ref{sec:experimental setup}.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{} See Figure \ref{fig:full main}.
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} See Sec. \ref{sec:experimental setup}.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{} See Sec. \ref{sec:experimental setup} and the readme file in the code submission.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> local_topology arxiv/sections/experiment.tex <==
%In this section, we compare \method{} and state-of-the-art methods under both full graph matching and partial graph matching settings.
In this section, we compare \method{} and state-of-the-art methods.
Due to the limited space, additional experimental results are provided in the appendix.

\begin{table}[tb]
	\centering
	\caption{\Datasets{} used in our experiments.}
	\label{tab:datasets}
	\begin{tabular}{lrrr}
		\toprule
		\textbf{Name}  & \textbf{Nodes} & \textbf{Edges} & \textbf{Description} \\
		\midrule
%		\textbf{Arenas Email} & 1,133 & 5,451 & communication network \\
		\textbf{PPI Yeast}   & 1,004  & 4,920   & protein-protein interaction network \\
		\textbf{Arxiv}            & 18,772  & 198,110 &  collaboration network    \\
		\textbf{LastFM ASIA} & 7,624 & 27,806 & social network  \\
		\bottomrule
	\end{tabular}
\end{table}

\subsection{Experimental Setup}\label{sec:experimental setup}

\paragraph{Computing infrastructure.}
All codes are implemented in Python 3.6 and the package dependencies are listed in the requirements.txt file in the code submission.
The experiments are conducted on a Ubuntu server with two CPUs (Intel Xeon (R) CPU E5-2680 v4 @ 2.40GHz), 4 Nvidia 2080 Ti graphics cards, and 378 GB of RAM.

\paragraph{Baselines.}
Our baselines are unsupervised methods including
(1) RefiNA \citep{heimann2021refining} that also explicitly considers the neighborhood consistency;
(2) REGAL \citep{heimann2018regal} that obtains the node embeddings based on matrix factorization;
(3) GRAMPA \citep{fan2020spectral} that is proposed to match correlated Erd\H{o}s-R\'{e}nyi graphs and involves computing all eigenvalues and the associated eigenvectors of the adjacency matrices;
(4) MM \citep{konar2020graph} that formulates graph matching as maximizing a monotone supermodular set function subject to matroid intersection constraints;
(5) GWL \citep{xu2019gromov} that matches graphs based on OT;
(6) GDD \citep{scott2021graph} that involves solving a three-level nested optimization problem.
As is shown in their papers, RefiNA and MM are sensitive to the noise and thus take the output of CONE-Align \citep{chen2020cone} as initialization.
For fair comparison, GWL and \method{} also use the output of CONE-Align to initialize the transport plan.
We implement REGAL, GWL, and GDD based on the corresponding open-sourced code.
%We implement REGAL \footnote{\url{https://github.com/GemsLab/REGAL}}, GWL \footnote{\url{https://github.com/HongtengXu/gwl}}, and GDD \footnote{\url{https://github.com/scottcb/DiffusionDistance}} based on the corresponding open-sourced code.

\paragraph{Evaluation Metric.}
We report node correctness ($\maNC$) that is defined as $\maNC=\frac{|\CM\cap\CM_{\mareal}|}{|\CM_{\mareal}|}$,
where $\CM$ and $\CM_{\mareal}$ are the learned and \groundtruth{} node correspondences respectively.


%For full matching, we calculate node correctness ($\maNC$) as $\maNC=\frac{|\CM\cap\CM_{\mareal}|}{|\CM_{\mareal}|}$ where $\CM$ and $\CM_{\mareal}$ are the learned and \groundtruth{} node correspondences respectively.
%For evaluation of partial graph matching,
%we compute the commonly used indicators including
%\begin{equation*}
%	\begin{aligned}
%		\recall&=\frac{\#\{\text{correct matching}\}}{\#\{\text{\groundtruth{} matching}\}},\\
%		\precision&=\frac{\#\{\text{correct matching}\}}{\#\{\text{total predicted matching}\}},\\
%		\Fone&=2\frac{\recall\cdot\precision}{\recall+\precision}.
%	\end{aligned}
%\end{equation*}




%We also empirically study the influence of different initializations in the Appendix.

%\paragraph{Key parameter choices.}

\subsection{Matching Permutated Networks}

\paragraph{\Datasets{}.}
Following the literature (eg. \citep{heimann2018regal,konar2020graph,heimann2021refining}), we match two randomly permutated graphs,
that is,
the target graph is obtained by permutating the nodes of the original graph (source graph).
\method{} is tested against baselines on standard benchmark \datasets{}, including
%Arenas Email \citep{kunegis2013konect},
PPI Yeast \citep{breitkreutz2007biogrid},
Arxiv \citep{leskovec2007graph},
and LastFM ASIA \citep{feather}.
These \datasets{} are listed in Table \ref{tab:datasets}.
Similar to \citet{heimann2018regal,konar2020graph,heimann2021refining},
we also add
structural noise to the target graph by adding $q|\EM^\src|$ edges.

%To extract partially overlapping subgraphs,
%we first determine the overlapped nodes, denoted by $\WM$.
%The rest of the nodes in the supergraph are split evenly into two sets $\UM^\src$ and $\UM^\tar$.
%The vertex sets are defined as $\VM^\src=\WM\cup\UM^\src$ and $\VM^\tar=\WM\cup\UM^\tar$ respectively.
%The overlap ratio is defined as $\rho=\frac{|\WM|}{\min\{|\VM^\src|,|\VM^\tar|\}}$.
%The edge set $\EM^\src$ (resp. $\EM^\tar$) consists of edges both of whose endpoints are in $\VM^\src$ (resp. $\VM^\tar$).
% isolated components?



\paragraph{Results.}
We report the performance of \method{} and baselines in Figure \ref{fig:full main},
in which $K$ is set to 3.
The similarity matrix in GRAMPA incurs quadruple computational complexity and takes thousands of hours to obtain on LastFM ASIA and Arxiv.
GRAMPA thus does not scale and its performance is not reported on these two \datasets{}.
OT-based methods and RefiNA take into account the local topology and have good performance on all \datasets{}.
\method{} outperforms state-of-the-art methods in all cases.
The improvement becomes more significant with the noise increasing.

\begin{figure}[ht]
	\centering
	\includegraphics[width=\textwidth]{imgs/full.pdf}
	\caption{NC of graph matching methods with $q|\EM^\src|$ noisy edges. The errorbars span 2 standard deviation. \method{} outperforms baselines on all \datasets{}.}\label{fig:full main}
\end{figure}


%\begin{figure}[ht]
%	\centering
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{imgs/full_yeast.pdf}
%		\caption{PPI Yeast}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{imgs/full_fm.pdf}
%		\caption{LastFM ASIA}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{imgs/full_arxiv.pdf}
%		\caption{Arxiv}
%	\end{subfigure}
%	\caption{NC of graph matching methods with $q|\EM^\src|$ noisy edges.}\label{fig:full main}
%\end{figure}

\paragraph{Runtime.}
\begin{table}[tb]
	\centering
	\caption{Average $\pm$ stdev runtime in sec of alignment methods from 5 trials.
		The two fastest methods per dataset are in bold.
		\method{} is faster than its closest competitors in accuracy (Figure \ref{fig:full main}).
	}
	\label{tab:full runtime}
	\begin{tabular}{lrrr}
		\toprule
		\textbf{Dataset}  & \textbf{PPI Yeast} & \textbf{LastFM ASIA} & \textbf{Arxiv} \\
		\midrule
		\textbf{GRAMPA} & 1985.895 $\pm$ 5.825 & / & / \\
		\textbf{REGAL} & 20.579 $\pm$ 0.844 & \textbf{210.842 $\pm$ 14.046} & \textbf{595.431 $\pm$ \quad 18.588}\\
		\textbf{MM} & 20.339 $\pm$ 0.576 & 430.333 $\pm$ 17.871 & 5424.995 $\pm$ \quad 29.580\\
		\textbf{GWL} & 110.682 $\pm$ 0.712 & 967.241 $\pm$ 13.372 & 35682.345 $\pm$ 1024.663\\
		\textbf{RefiNA} & \textbf{17.887 $\pm$ 0.209} & 344.009 $\pm$\,\,\, 8.475 & 3115.087	$\pm$ \quad 74.360 \\
		\textbf{GDD} & 54.666 $\pm$ 1.684 & 6732.156 $\pm$	10.883 & 125965.441 $\pm$	1383.409 \\
		\midrule
		
		\textbf{\method{}} & \textbf{9.731 $\pm$ 0.417} & \textbf{131.241 $\pm$\,\,\, 1.249} & \textbf{2011.765 $\pm$ \quad 15.081} \\
		
		\bottomrule
	\end{tabular}
\end{table}

In Table \ref{tab:full runtime}, we compare the average runtimes of all different methods across noise levels.
Time used to calculate the heat diffusion wavelets in \method{} is included.
The two fastest
methods per dataset are in bold.
 \method{} is faster
than its closest competitors in accuracy (Figure \ref{fig:full main}).



%\subsection{Partial Graph Matching}
%
%\paragraph{Results.}
%
%\paragraph{Runtime.}



==> local_topology arxiv/sections/introduction-v1.tex <==
Graph matching (network alignment) aims to identify the correspondence of nodes across two related graphs,
by minimizing the sum of pair-wise matching costs of corresponding nodes/edges.
It has many applications,
such as
linking user accounts in social platforms \citep{shu2017user,wang2019user},
aligning entities in knowledge graphs \citep{sun2020knowledge,pei2020rea},
and matching keypoints across two images \citep{sarlin2020superglue,wang2020zero},
to name a few.

%The choice of matching costs is critical to the performance of graph matching.%when side available，设计matching costs更加困难如果只有拓扑连接，
%Originally, matching costs are mainly calculated using handcrafted features that rely%不要mainly
%heavily on expert knowledge \citep{patro2012global,sun2015simultaneous,mamano2017sana}.
%Recently, end-to-end deep learning methods for graph matching are proposed
%to automatically learn the node embedding-based matching
%costs \citep{zanfir2018deep,fey2019deep,wang2019learning,sarlin2020superglue,wang2020combinatorial}.
%These methods, however, require side information including node or edge features, and a large amount of anchor links (labelled node correspondences).
%In practice, side information are often not available \citep{snapnets,heimann2021refining}.%however in many tasks，没有side information使得更加复杂更难，只能通过
%Under such circumstance,
%the node correspondence is often estimated on the sole basis of the network topologies of the two graphs.%连接关系，后面这句是主句。

The choice of matching costs is critical to the performance of graph matching.
%and designing matching costs is more challenging when node or edge features are not available.
When  node/edge side information, e.g. attributes, are available,
one can rely on expert knowledge to design handcrafted node embeddings for the calculation of matching costs
% matching costs are commonly calculated by using handcrafted features that rely heavily on expert knowledge 
\citep{zhang2016final,meng2016igloo}.
Recently, to alleviate the requirement of expert knowledge, 
end-to-end deep learning methods are proposed
to learn the node embedding automatically based on the \emph{anchor links} (labelled node correspondences)\citep{zanfir2018deep,fey2019deep,wang2019learning,sarlin2020superglue,wang2020combinatorial}.
However, in many tasks, side information and/or anchor links are not available \citep{snapnets,heimann2021refining}.
Under such circumstance,
These methodshowever, require side information including node or edge features, and a large amount of \emph{anchor links} (labelled node correspondences).
In many tasks, however, graphs are often unattributed \citep{snapnets,heimann2021refining}.
Under such circumstance,
the matching costs are often estimated on the sole basis of the network topologies of the two graphs.

%\citeauthor{heimann2021refining} \citeyear{heimann2021refining} theoretically demonstrates a close relationship between \emph{matched neighborhood consistency} (MNC) and the matching quality.
The seminal work of \citet{heimann2021refining} reveals the close connection between \emph{matched neighborhood consistency} (MNC) and the alignment accuracy.
In particular,
accurate alignment entails high MNC.
However, several limitations still remain:%紧密的关系，connection between
1) Their method, RefiNA, only considers the numerators of MNC values, which leads to a gap between their method and their theoretical analysis;
2) RefiNA only uses one-hop neighborhoods, which easily leads to (near) structural indistinguishability and misaligns nodes that have low degrees.

Recently, one line of works align graphs by borrowing tools from
optimal transport (OT),
which can match graphs in an unsupervised fashion \citep{memoli2011gromov,maretic2019got,xu2019gromov,titouan2019optimal,chowdhury2019gromov,barbe2020graph}.
These methods exploit the geometric properties of the metric spaces that underlie the graphs and exhibits good empirical performance.
Basically, the node correspondence is estimated by calculating the \emph{transport plan} of the Gromov-Wasserstein distance that captures the \emph{global} structural information \citep{barbe2020graph}.
However, it remains unknown how these OT-based methods exploit the \emph{local} topology to iteratively improve the matching accuracy and whether they conform to the MNC principle.
Besides, their alignment costs hinge on the one-hop neighborhood of each node, which leaves room for improvement.

%Recently, there has been significant interest in designing \emph{heat diffusion}-based methods to capture the structural information of graphs (eg. \citep{tsitsulin2018netlsd,berberidis2018adaptive,donnat2018learning,klicpera2019diffusion}). 
%The heat diffusion on a graph is the solution to the discrete heat equation \citep{kondor2002diffusion}.
%Intuitively, each node propagates a unit of energy over the graph and the local topology is characterized by the amount of energy that each neighboring node receives after a given time.
%It can be proved that nodes that share similar local topology have similar diffusion patterns \citep{donnat2018learning}.
%which also implies that heat diffusion is robust to small perturbations of the edge structure \citep{donnat2018learning,berberidis2018adaptive,klicpera2019diffusion}.
%The computational complexity of heat diffusion is linear in the number of edges \citep{defferrard2016convolutional,donnat2018learning}, thus allowing it to scale to \realworld{} graphs.
%Therefore, heat diffusion allows us to characterize the multi-hop neighborhood of each node and match node pairs that have similar local topological structures.
%Heat diffusion, however, is mainly used to fuse node attributes in attributed graphs instead of matching unattributed graphs in the graph matching literature \citep{li2019graph,barbe2020graph}.


%In this paper, we propose a novel graph matching method \method{} to tackle the challenging problem of matching two unattributed graphs without anchor links.
%Our method uses \emph{heat diffusion wavelet} (HDW) \citep{donnat2018learning} to characterize the structure of multi-hop neighborhoods (hence the name).
%Based on the captured structural information,
%we define a novel quantity, pairwise \si{} (\sis{}).%先提这个概念，比measure更弱的量criterion，揭示了和accuracy的关系。提出了新方法。可以很容易嵌入小波
%Our method improves the alignment scores of node pairs that have low \sis{} values in each iteration.

This paper considers the challenging problem of matching two unattributed graphs without anchor links.
A novel concept, \si{} (\sis{}), is defined to measure the correspondence quality of a node pair.
We reveal the connection between \sis{} values of predicted node counterparts and the matching quality.
Our method, \method{}, improves the alignment scores of node pairs that have low \sis{} values in each iteration.
By incorporating \emph{heat diffusion wavelet} \citep{donnat2018learning},
\method{} considers the multi-hop structural information and increases the distinguishability of nodes.

%Our contributions are summarized as follows.
%\begin{itemize}
%	\item \textbf{A new method.}%更符合，并且引入k.
%	A novel quantity, pairwise \si{} (\sis{}), is defined to evaluate the quality of the estimated node correspondence,
%	based on which we propose a new graph matching method named \method{}.
%	By taking a larger neighborhood into account,
%	the (near) structural indistinguishability problem is alleviated.
%	\item \textbf{Theoretical analysis.}% corresponding SI 和MNC的关系，理论分析要有形容词，对应关系
%	We theoretically analyze the relationship between \sis{} and the alignment accuracy.
%	We prove that \method{} can reduce \sis{} under suitable assumptions.
%	The convergence of \method{} to a first-order stationary point is proved and the true matching matrix is proved to be one fixed point of the update.
%	We demonstrate that our method is essentially the mirror descent method for solving the Gromov-Wassetstein distance and thus provides a local topological perspective for OT-based methods.
%	We also reveal that our method increases a lower bound of MNC values.
%\end{itemize}

Our contributions are summarized as follows.
\begin{itemize}
	\item We propose a new graph matching method named \method{} to match two unattributed graphs without anchor links.
	Compared to RefiNA \citep{heimann2021refining},
	\method{} is more conforming to the MNC principle.
	By taking a larger neighborhood into account,
	\method{} increases the distinguishability of nodes and improves the matching quality.
	\item We conduct theoretical analysis for \method{}.
	We reveal that \sis{} have a close relationship to matching accuracy.
	On the one hand, if a pair of nodes incurs zero \sis{}, they have the same local topology.
	On the other hand, \sis{} values of true counterparts are bounded and close to zero.
	Under suitable assumptions, \method{} can reduce \sis{} values of true counterparts.
	We demonstrate that \method{} is essentially a mirror descent method for solving the Gromov-Wassetstein distance and provides a local topological perspective for OT-based methods.
	We also prove that our method increases a lower bound of MNC values, instead of increasing the numerators.
\end{itemize}

Extensive experimental results demonstrate that the proposed method outperforms state-of-the-art methods.
The rest of the paper is organized as follows.
In Sec. \ref{sec:preliminary}, we review the background and discuss the relationship between \sis{} and matching accuracy.
Based on \sis{}, a new graph matching method \method{} is proposed in Sec. \ref{sec:method}.
We give theoretical analysis in Sec. \ref{sec:theory}.
Due to the limited space, all proof are given in the appendix.
Experimental results are demonstrated in Sec. \ref{sec:experiment} and the appendix.



%Graph matching is a key step for many graph analysis tasks including
%%	graph isomorphism test \citep{mckay1981practical,aflalo2015convex},
%graph clustering \citep{titouan2019optimal,xu2020gromov},
%graph classification \citep{titouan2019optimal,vincent2021online},
%graph generation \citep{xu2020gromov},
%and network retrieval \citep{berretti2001efficient,ozer2002graph}.
%It also has applications to many problems of industrial or academic interest, such as
%linking user accounts in social platforms \citep{shu2017user,wang2019user},
%entity alignment in knowledge graphs \citep{sun2020knowledge,pei2020rea},
%and matching keypoints across two images \citep{sarlin2020superglue,wang2020zero},
%to name a few.




==> local_topology arxiv/sections/introduction.tex <==
Graph matching (network alignment) aims to identify the correspondence of nodes across two related graphs,
by minimizing the sum of pair-wise matching costs of corresponding nodes/edges.
It has many applications,
such as
linking user accounts in social platforms \citep{shu2017user,wang2019user},
aligning entities in knowledge graphs \citep{sun2020knowledge,pei2020rea},
and matching keypoints across two images \citep{sarlin2020superglue,wang2020zero},
to name a few.

%The choice of matching costs is critical to the performance of graph matching.%when side available，设计matching costs更加困难如果只有拓扑连接，
%Originally, matching costs are mainly calculated using handcrafted features that rely%不要mainly
%heavily on expert knowledge \citep{patro2012global,sun2015simultaneous,mamano2017sana}.
%Recently, end-to-end deep learning methods for graph matching are proposed
%to automatically learn the node embedding-based matching
%costs \citep{zanfir2018deep,fey2019deep,wang2019learning,sarlin2020superglue,wang2020combinatorial}.
%These methods, however, require side information including node or edge features, and a large amount of anchor links (labelled node correspondences).
%In practice, side information are often not available \citep{snapnets,heimann2021refining}.%however in many tasks，没有side information使得更加复杂更难，只能通过
%Under such circumstance,
%the node correspondence is often estimated on the sole basis of the network topologies of the two graphs.%连接关系，后面这句是主句。

The choice of matching costs is critical to the performance of graph matching.
%and designing matching costs is more challenging when node or edge features are not available.
When  node/edge side information, e.g. attributes, is available,
one can rely on expert knowledge to design handcrafted node embeddings for the construction of matching costs
% matching costs are commonly calculated by using handcrafted features that rely heavily on expert knowledge 
\citep{zhang2016final,meng2016igloo}.
Recently, to alleviate the requirement of expert knowledge, 
end-to-end deep learning methods are proposed
to learn the node embedding automatically based on the \emph{anchor links} (labelled node correspondences) \citep{zanfir2018deep,fey2019deep,wang2019learning,sarlin2020superglue,wang2020combinatorial}.
However, in many tasks, side information may not be available\citep{snapnets,heimann2021refining}.
Under such circumstance,
the matching costs can merely be estimated on the basis of the network topologies of the two graphs \citep{patro2012global,saraph2014magna,sun2015simultaneous,memoli2011gromov,maretic2019got,xu2019gromov,heimann2021refining}.

Among these network-topology based methods,
one line of works align graphs by borrowing tools from optimal transport (OT) and achieve the state-of-the-art performance  \citep{memoli2011gromov,maretic2019got,xu2019gromov,titouan2019optimal,chowdhury2019gromov,barbe2020graph}.
Basically, these methods utilize OT to exploit the geometric properties of the metric spaces that underlie the graphs, 
and  estimate the node correspondence by calculating the \emph{transport plan} of the Gromov-Wasserstein distance. 
Typically, the matching costs in these methods are calculated depending on the one-hop neighborhood information of each node.
%and then utilize OT to exploit the geometric properties of the metric spaces that underlie the graphs.
%The node correspondence is estimated by calculating the \emph{transport plan} of the Gromov-Wasserstein distance.
%Besides, their alignment costs hinge on the one-hop neighborhood of each node, which leaves room for improvement.


%\citeauthor{heimann2021refining} \citeyear{heimann2021refining} theoretically demonstrates a close relationship between \emph{matched neighborhood consistency} (MNC) and the matching quality.
Recently, \citet{heimann2021refining} reveals the connection between the graph matching accuracy and the  \emph{matched neighborhood consistency} (MNC), i.e., the Jaccard simliarity between the one-hop neighborhoods of matched node pairs.
In particular, they show that accurate matching essentially entails high MNC.
However, it remains unknown how the OT-based methods  are related to MNC theoretically.
Instead, they propose a method, RefiNA, by maximizing the numerators of MNC, which can be regarded as an opposite measure of the matching cost.
%aims to increase the MNC. 
Though the authors intend to find matching with high MNC, RefiNA actually diverges from their purpose, as the denominator of MNC is ignored and a high numerator does not ensure a high MNC.
Moreover, both OT-based methods and RefiNA may suffer from one-hop structural indistinguishability and tend to misalign nodes that have low degrees, as they discard the abundant network topological information and estimate the graph matching merely depending on the one-hop neighborhoods structure.



%This paper considers the challenging problem of matching two unattributed graphs without anchor links.
In this paper, we propose a novel criterion to measure the graph matching accuracy, \emph{\si{}} (\sis{}), which utilizes the abundant network topological information.
Specifically, \sis{} incorporates the \emph{heat diffusion wavelet} \citep{donnat2018learning} to  accommodate the multi-hop structure of the graphs.
If a pair of nodes incurs zero \sis{}, they are $K$-hop indistinguishable.
On the other hand, \sis{} values of true counterparts should be zero for two isomorphic graphs.
In practice, the \sis{} between a true corresponding pairs may only close to 0 due to the structural noise.

%is defined to measure the correspondence quality of a node pair.
%We reveal the connection between \sis{} values of predicted node counterparts and the matching quality.
Based on \sis{}, we propose a \emph{Structural Inconsistency reducing Graph Matching Algorithm} (SIGMA),
which improves the alignment scores of node pairs that have low \sis{} values in each iteration.
Under suitable assumptions, \method{} can reduce \sis{} values of true counterparts.
As \sis{} considers the multi-hop topological information, \method{} can avoid the misguidance of one-hop structural indistinguishability and find graph matching of higher accuracy.
Besides, we also show that our method increases a soft version of MNC values, which is positively related to MNC and should also be high/low for accurate/inaccurate matching.
Furthermore, we demonstrate that \method{} can be derived by using a mirror descent method to solve the Gromov-Wasserstein distance with a novel $K$-hop-structure-based  matching costs.
As a result, \method{} can be regarded as the first OT-based method that are guaranteed to increase MNC in each iteration in the graph matching literature.



Extensive experimental results demonstrate that the proposed method outperforms state-of-the-art methods.
The rest of the paper is organized as follows.
In Sec. \ref{sec:preliminary}, we review the background and discuss the relationship between \sis{} and matching accuracy.
Based on \sis{}, a new graph matching method \method{} is proposed in Sec. \ref{sec:method}.
We give theoretical analysis in Sec. \ref{sec:theory}.
Due to the limited space, all proof are given in the appendix.
Experimental results are demonstrated in Sec. \ref{sec:experiment} and the appendix.



%Graph matching is a key step for many graph analysis tasks including
%%	graph isomorphism test \citep{mckay1981practical,aflalo2015convex},
%graph clustering \citep{titouan2019optimal,xu2020gromov},
%graph classification \citep{titouan2019optimal,vincent2021online},
%graph generation \citep{xu2020gromov},
%and network retrieval \citep{berretti2001efficient,ozer2002graph}.
%It also has applications to many problems of industrial or academic interest, such as
%linking user accounts in social platforms \citep{shu2017user,wang2019user},
%entity alignment in knowledge graphs \citep{sun2020knowledge,pei2020rea},
%and matching keypoints across two images \citep{sarlin2020superglue,wang2020zero},
%to name a few.




==> local_topology arxiv/sections/methodology.tex <==
Motivated by our perspective, we propose a new graph matching algorithm \method{}.
Crucial details are discussed in this section.
%We present the proposed \method{} in Algorithm \ref{alg:method} and discuss about some crucial details in this section.




\subsection{Objective Function}


Assuming $|\VM^\src|\le|\VM^\tar|$, graph matching aims to find an injective mapping $\pi:\VM^\src\to\VM^\tar$ that matches nodes in $\GM^\src$ to nodes in $\GM^\tar$.
$\pi$ is also commonly represented as a matching matrix $\TB=\{0,1\}^{|\VM^\src|\times |\VM^\tar|}$,
where $T_{ii'}=1$ if node $i$ in $\GM^\src$ is matched to node $i'$ in $\GM^\tar$, and $T_{ii'}=0$ otherwise (eg. \citep{fey2019deep,heimann2021refining}).
%Assuming $\GM^\src$ has fewer or equal number of nodes than $\GM^\tar$ without loss of generality $|\VM^\src|\le|\VM^\tar|$, 
We find the matching matrix by solving the following quadratic assignment problem
\begin{equation}\label{eq:discrete formulation}
	\min_{\TB\in\PM^f}\sum_{i=1}^{|\VM^\src|}\sum_{j=1}^{|\VM^\src|}\sum_{i'=1}^{|\VM^\tar|}\sum_{j'=1}^{|\VM^\tar|}d_{ii'jj'}T_{ii'}T_{jj'},
\end{equation}
where $d_{ii'jj'}$ is the cost for the pairwise assignment $(i,j)\rightarrow (i',j')$,
and the feasible domain is
\begin{equation*}
	\PM^f=\Big\{\TB\in\{0,1\}^{|\VM^\src|\times |\VM^\tar|}\Big|\TB\oneB=\oneB,\TB^\top\oneB\le\oneB\Big\},
\end{equation*}
where $\oneB$ is an all-ones vector.

Compared to \citep{xu2019gromov,xu2019scalable} that only use edge weights to define the alignment costs,
the cost $d_{ii'jj'}$ of \method{} exploits the local topological structure.
The $K$-th order heat diffusion wavelet allows us to define a new matrix $\BB^z=[B_{ij}^z]$ describing node dissimilarities within each graph, i.e.,
\begin{equation}
	B_{ij}^z=\begin{cases}
		&\bar{\Psi}-\Psi_{ij}^z,\text{ if }i\neq j,\\
		&0, \text{ else,}
	\end{cases}
\end{equation}
where $\Psi_{ij}^z$ is defined as Eq. (\ref{eq:heat diffusion wavelet}), $z=\src,\tar$ and constant $\bar{\Psi}>\max_{i,j,z}\Psi_{ij}^z$.
%Obviously, $B_{ij}^z=\bar{\Psi}$ if node $j$ is more than $K$ hops away from node $i$ and $\BB^z$ measures the local topology of each node.
The alignment cost incorporating the local topological structure is thus defined as $d_{ii'jj'}=(B_{ij}^\src-B_{i'j'}^\tar)^2$.

%Such formulation matches every node in $\GM^\src$ to a node in $\GM^\tar$ and hence is referred to as \emph{full matching} \citep{kazemi2015can}.
%In real-world applications, $\GM^\src$ and $\GM^\tar$ are often two partially overlapping subgraphs of an underlying supergraph, that is, some nodes in one graph may not
%exist in the other one.
%Thus, our method also considers \emph{partial matching} by replacing the constraint $\PM^f$ with $\PM^p$ given by
%\begin{equation*}
%	\PM^p=\Big\{\TB\in\{0,1\}^{|\VM^\src|\times |\VM^\tar|}\Big|\TB\oneB\le\oneB,\TB^\top\oneB\le\oneB, \oneB^\top\TB\oneB=b\Big\},
%\end{equation*}
%where $b\le\min\{|\VM^\src|,|\VM^\tar|\}$.
%When the equality holds, partial matching is reduced to full matching.

\subsection{Optimization}\label{sec:optimization}
By relaxing $\TB\in\{0,1\}^{|\VM^\src|\times |\VM^\tar|}$ to $\TB\in[0,1]^{|\VM^\src|\times |\VM^\tar|}$,
Problem (\ref{eq:discrete formulation}) is converted to solving the partial GW discrepancy
\begin{equation}\label{eq:continuous formulation}
	\min_{\TB\in\Pi^{|\VM^\src|}}\ell(\TB):=\sum_{i=1}^{|\VM^\src|}\sum_{j=1}^{|\VM^\src|}\sum_{i'=1}^{|\VM^\tar|}\sum_{j'=1}^{|\VM^\tar|}d_{ii'jj'}T_{ii'}T_{jj'},
\end{equation}
where $\Pi^{|\VM^\src|}=\{\TB\in[0,1]^{|\VM^\src|\times |\VM^\tar|}\Big|\TB\oneB=\oneB,\TB^\top\oneB\le\oneB, \oneB^\top\TB\oneB=|\VM^\src|\}$,
since we assume $|\VM^\src|\le|\VM^\tar|$.

The most common algorithm for solving Problem (\ref{eq:continuous formulation}) is gradient descent that iteratively updates $\TB$ as follows
\begin{equation}\label{eq:gd}
	\TB^{(\tau+1)}=\proj_{\Pi^{|\VM^\src|}}\Big\{\TB^{(\tau)}-\eta^{(\tau)}\nabla \ell(\TB^{(\tau)})\Big\}.
\end{equation}

Mirror descent takes into account the geometry of the feasible domain \citep{bubeck2015convex}, and is better-suited to Problem (\ref{eq:continuous formulation}).
Mirror descent is given by the recurrence
\begin{equation}\label{eq:md 0}
	\TB^{(\tau+1)}=\argmin_{\TB\in\Pi^{|\VM^\src|}}\langle \nabla \ell(\TB^{(\tau)}),\TB\rangle+\frac{1}{\eta^{(\tau)}}D_\psi(\TB,\TB^{(\tau)}),
\end{equation}
where $D_\psi(\TB,\TB^{(\tau)})$ stands for the Bregman divergence.
%where $D_\psi(\TB,\TB^{(\tau)})=\psi(\TB)-\psi(\TB^{(\tau)})-\langle\nabla\psi(\TB^{(\tau)}),\TB-\TB^{(\tau)}\rangle$ stands for the Bregman divergence generated by a strongly convex and continuously differentiable function $\psi(\TB)$.
When one selects KL-divergence as the Bregman divergence,
(\ref{eq:md 0}) becomes
\begin{equation}\label{eq:md}
	\TB^{(\tau+1)}=\proj_{\Pi^{|\VM^\src|}}\Big\{\TB^{(\tau)}\odot\exp\big(-\JB-\eta^{(\tau)}\nabla\ell(\TB^{(\tau)})\big)\Big\},
\end{equation}
where $\JB$ is the all-ones matrix, $\odot$ is the element-wise multiplication, and the exponentiation is also element-wise.
%Adopting the aforementioned assignment costs, the gradient has the following form,
%\begin{equation}\label{eq:gradient}
%	\nabla\ell(\TB)=h(\BB^\src)\oneB\otimes\pB+\oneB\otimes h(\BB^\tar)\qB-2\BB^\src\TB^{(\tau)}\BB^\tar
%\end{equation}
%where $\pB=\TB\oneB$, $\qB=\TB^\top\oneB$, $h$ denotes the element-wise square and $\otimes$ is the outer product of two vectors \citep{peyre2016gromov}.

If the projections in Eq. (\ref{eq:gd}) and (\ref{eq:md}) are based on the KL-divergence, they can be solved via periodic projections \citep{benamou2015iterative}.
\method{} converges to an $\epsilon$-stationary point with the number of mirror descent iterations $\OM(\frac{1}{\epsilon^2})$,
by Corollary 3.1 of \citet{zhang2018convergence}.
%Let $\CM_1=\{\TB|\TB\oneB\le\oneB\}$, $\CM_2=\{\TB|\TB^\top\oneB\le\oneB\}$, and $\CM_3=\{\TB|\oneB^\top\TB\oneB=|\VM^\src|\}$.
%The KL-divergence based projection onto these three sets have closed forms
%\begin{equation}\label{eq:periodic projections}
%	\begin{aligned}
%		\proj_{\CM_1}^\KL(\TB)&=\Diag\Big(\min\{\frac{\oneB}{\TB\oneB},\oneB\}\Big)\TB,\\
%		\proj_{\CM_2}^\KL(\TB)&=\Diag\Big(\min\{\frac{\oneB}{\TB^\top\oneB},\oneB\}\Big)\TB,\\
%		\proj_{\CM_3}^\KL(\TB)&=\TB\frac{|\VM^\src|}{\oneB^\top\TB\oneB},
%	\end{aligned}
%\end{equation}
%where the division and minimum is element-wise.
%Extending the indexing of the sets by $3$-periodicity so that they satisfy $\CM_{k+3}=\CM_k$ for all $k\in\NBB$, one computes $\forall k>0$, $\TB^{(k,\tau)}=\proj_{\CM_k}^\KL(\TB^{(k-1,\tau)})$ with $\TB^{(0,\tau)}=\TB^{(\tau)}\odot\exp\big(-\JB-\eta^{(\tau)}\nabla\ell(\TB^{(\tau)})\big)$.
%%%%%%%%%%%%%%%  new description  %%%%%%%%%%%%%%%%%%%%%%
%A periodic sequence $\{\CM_k|k>0 \text{ and }k\in\NBB\}$ is constructed so that they satisfy $\CM_{k+3}=\CM_k$ for all positive integers $k$,
%where $\CM_1=\{\TB|\TB\oneB\le\oneB\}$, $\CM_2=\{\TB|\TB^\top\oneB\le\oneB\}$, and $\CM_3=\{\TB|\oneB^\top\TB\oneB=|\VM^\src|\}$.
%For all $k>0$, one computes $\TB^{(k,\tau)}=\proj_{\CM_k}^\KL(\TB^{(k-1,\tau)})$ with $\TB^{(0,\tau)}=\TB^{(\tau)}\odot\exp\big(-\JB-\eta^{(\tau)}\nabla\ell(\TB^{(\tau)})\big)$.
%The KL-divergence based projection onto these three sets have closed forms
%\begin{equation}\label{eq:periodic projections}
%	\begin{aligned}
%		\proj_{\CM_1}^\KL(\TB)&=\Diag\Big(\min\{\frac{\oneB}{\TB\oneB},\oneB\}\Big)\TB,\\
%		\proj_{\CM_2}^\KL(\TB)&=\TB\Diag\Big(\min\{\frac{\oneB}{\TB^\top\oneB},\oneB\}\Big),\\
%		\proj_{\CM_3}^\KL(\TB)&=\TB\frac{|\VM^\src|}{\oneB^\top\TB\oneB},
%	\end{aligned}
%\end{equation}
%where the division and minimum is element-wise.
%The following proposition states the convergence of periodic projections.
%\begin{proposition}[Proposition 5 of \citet{benamou2015iterative}]
%	$\TB^{(k,\tau)}$ converges towards the unique projection $\argmin_{\TB\in\PM^p}\KL(\TB\|\TB^{(0,\tau)})$.
%\end{proposition}

%\method{} updates the transport plan as (\ref{eq:md}).
%The convergence is guaranteed as follows and the proof is given in the appendix.
%\begin{proposition}[Corollary 3.1 of \citet{zhang2018convergence}]\label{prop:md}
%	\method{} converges to an $\epsilon$-stationary point with the number of mirror descent iterations $\OM(\frac{1}{\epsilon^2})$.
%\end{proposition}

\paragraph{Computational complexity.}
The complexity for calculaing the heat diffusion wavlets is $\OM(KV^3)$ where $V=\max\{|\VM^\src|,|\VM^\tar|\}$.
Due to the two matrix multiplication steps of the term $\BB^\src\TB\BB^\tar$,
calculating the gradient involves computational complexity $\OM(V^3)$.
Note that the matrix multiplication is highly parallelizable and well-suited to modern computing architectures like GPUs.
$\OM(V^2)$ cost is induced by periodic projections.
Therefore, if we run projected mirror descent for $N$ iterations, each of which has $T$ periodic projections,
$\OM\big(NTV^2+(N+K)V^3\big)$ computational cost is required in learning the optimal transport.
Such complexity is of the same order as state-of-the-art methods like \citet{xu2019gromov,konar2020graph,scott2021graph,heimann2021refining},
and lower than \citet{neyshabur2013netal,malod2015graal,fan2020spectral}.
Considering the sparsity of edges in \realworld{} graphs,
the complexity can be reduced to $\OM\big(NTV^2+(N+K)VE\big)$ where $E=\max\{|\EM^\src|,|\EM^\tar|\}$.

%To further reduce the computational complexity and memory footprint,
%we can recursively partition graphs into aligned sub-graph pairs,
%across which the node correspondence can be found by \method{} (just as techniques proposed in \citep{xu2019scalable}).
%The time and memory complexity are reduced to $\OM\big(N(E+V)\log V+NTV^2\big)$ and $\OM(E+V)$, where $E=\max\{|\EM^\src|,|\EM^\tar|\}$.
%Note that directly partitioning graphs like \citet{xu2019scalable} modifies the local topology of many nodes and thus hurts the alignment accuracy.
%By precomputing and storing the local topological information in $\BB^z$, such problem is overcome.




\begin{algorithm}[ht]
	\caption{\method{} \label{alg:method}}
	\begin{algorithmic}[1]
		\State {\textbf{Input:}} Total rounds $T$, graphs $\GM^\src$ and $\GM^\tar$, initial transport plan $\TB^{(0)}$.
		\State {\textbf{Output:}} Correspondence set $\CM$.
		\State Calculate and store matrices $\BB^\src$ and $\BB^\tar$.
		\For{$\tau=0,\dots,T-1$}
		\State Update $\TB^{(\tau+1)}$ by iteration \ref{eq:md}.
		\EndFor
		\State $\tilde{\TB}=\TB^{(T)}$
		\State Initialize correspondence set $\CM=\emptyset$
		\For{$i\in\VM^\src$}
		\State $i'=\arg\max_{i'} \tilde{T}_{ii'}$.
		\State $\CM=\CM\cup\{(i,i')\}$
		\EndFor
	\end{algorithmic}
\end{algorithm}

\method{} is summarized in Algorithm \ref{alg:method}.
The matching cost is based on heat diffusion wavelets.
It updates the transport plan using mirror descent.
By choosing the largest $\tilde{T}_{ii'}$ for each i, we find the correspondence.

%\begin{algorithm}[ht]
%	\caption{\method{} \label{alg:method}}
%	\begin{algorithmic}[1]
%		\State {\textbf{Input:}} Total rounds $T$, graphs $\GM^\src$ and $\GM^\tar$, matrices $\BB^\src$ and $\BB^\tar$, and total transport mass $b$.
%		\State {\textbf{Output:}} Correspondence set $\CM$.
%		\State Randomly initialize $\TB_0\in\PM^p$.\Comment{If $b<|\VM^\src|$, \method{} conducts partial matching.}
%		%		\State Calculate and store heat diffusion wavelets.
%		\For{$\tau=0,\dots,T-1$}
%		\State Update $\TB_{\tau+1}$ by iteration \ref{eq:mirror descent}.
%		\EndFor
%		\State $\tilde{\TB}=[\TB_T,\oneB-\TB_T\oneB]$\Comment{The extended transport plan $\tilde{\TB}\in\RBB^{|\VM^\src|\times(|\VM^\tar|+1)}$.}
%		\State Initialize correspondence set $\CM=\emptyset$
%		\For{$i\in\VM^\src$}
%		\State $i'=\arg\max_{i'} \tilde{T}_{ii'}$.
%		\If{$i'\neq(|\VM^\tar|+1)$}\Comment{Otherwise, $i$ is matched to the dummy point.}
%		\State $\CM=\CM\cup\{(i,i')\}$
%		\EndIf
%		\EndFor
%	\end{algorithmic}
%\end{algorithm}
%
%\method{} is summarized in Algorithm \ref{alg:method}.
%We use the learned $\TB_T$ to construct an extended transport plan $\tilde{\TB}=[\TB_T,\oneB-\TB_T\oneB]\in\RBB^{|\VM^\src|\times(|\VM^\tar|+1)}$.
%This can be thought of adding a \emph{dummy} point to $\GM^\tar$, which is similar to \citep{chapel2020partial}.
%By choosing the largest $\tilde{T}_{ii'}$ for each i, we find the correspondence.

\subsection{Topological interpretation}\label{sec:interpretation}
%The key principle for matching undirected and unattributed graphs is the topological consistency:
%nodes that are close in one graph should be matched to nodes that are close in the other graph \citep{heimann2021refining}.
%\method{} achieves the topological consistency by using assignment costs that quantify the local topological consistency,
%which we formulate in this subsection.

Adopting the aforementioned assignment costs, the gradient has the following form,
\begin{equation}\label{eq:gradient}
	\nabla\ell(\TB)=h(\BB^\src)\oneB\otimes\pB+\oneB\otimes h(\BB^\tar)\qB-2\BB^\src\TB^{(\tau)}\BB^\tar
\end{equation}
where $\pB=\TB\oneB$, $\qB=\TB^\top\oneB$, $h$ denotes the element-wise square and $\otimes$ is the outer product of two vectors \citep{peyre2016gromov}.
Substituting Eq. (\ref{eq:gradient}) into the mirror descent update \ref{eq:md},  Eq. (\ref{eq:md}) can be rewritten as
\begin{equation}\label{eq:mirror descent}
	\TB^{(\tau+1)}=\proj_{\Pi^{|\VM^\src|}}\Big(\frac{1}{e}\TB^{(\tau)}\odot\SB(\TB)^{\eta(\tau)}\Big),
\end{equation}
where $\SB(\TB)=\exp\Big(2\BB^\src\TB\BB^\tar-h(\BB^\src)\pB\otimes\oneB-\oneB\otimes h(\BB^\tar)\qB\Big)$ and the exponentiation is element-wise.

When $K=1$, the topology violation has a more intuitive interpretation.
\begin{proposition}\label{prop:relationship with MNC}
	When one only uses one-hop neighborhood information (i.e., $K=1$) to match two graphs of the same number of nodes,
	\begin{equation*}
		\begin{aligned}
			\exp\big(-d(i,i';\TB)\big)=\frac{\exp\Big(t|\tilde{\NM}_1^\src(i;\pi)\cap\NM_1^\tar(i')|\Big)}{\exp\Big(t|\tilde{\NM}_1^\src(i;\pi)\cup\NM_1^\tar(i')|\Big)},
		\end{aligned}
	\end{equation*}
	where $\TB\in\PM^f$, $\tilde{\NM}_k^\src(i;\pi)=\{j'\in\VM^\tar|\exists j\in\NM_k^\src(i) \st \pi(j)=j'\}$, and the bijective is given by $\pi(i)=\argmax_{i'}T_{ii'}$.
	Compared to $\operatorname{MNC}(i, i';\pi)=\frac{\left|\tilde{\NM}_1^{\src}(i;\pi) \cap \NM_{1}^\tar(i')\right|}{\left|\tilde{\NM}_1^{\src}(i;\pi) \cup \NM_{1}^\tar(i')\right|}$ \citep{chen2020cone,heimann2021refining},
	$\exp\big(-d(i,i';\TB)\big)\le\MNC(i,i';\pi)$ when $t=1$ and $\tilde{\NM}_1^{\src}(i;\pi) \cap \NM_{1}^\tar(i')$ is not empty.
\end{proposition}


%The transport distance between the heat diffusion wavelet coefficients,
%$d(i,i';\TB)=\sum_{j=1}^{|\VM^\src|}\sum_{j'=1}^{|\VM^\tar|}T_{jj'}(B_{ij}^\src-B_{i'j'}^\tar)^2$,
%measures the topology violation between nodes $i$ and $i'$ for matching matrix $\TB$.
%Based upon $d(i,i';\TB)$, we can define the \emph{\Quantity} (\Quan{}) that measures the topological consistency of node $i$ and node $i'$ given matching matrix $\TB$ as\footnote{Defining similarity values based on distance functions is common in machine learning literature. For example, in \citet{hinton2002stochastic,van2008visualizing}, the similarity value between two embedding vectors $\zB_i$ and $\zB_j$ with distance $d(\zB_i,\zB_j)$ is defined as $\exp\big(-d(\zB_i,\zB_j)\big)$.}
%\begin{equation}
%	\maQuan(i,i';\TB)=e^{-d(i,i';\TB)}.
%\end{equation}

%Eq. (\ref{eq:mirror descent}) implies that each iteration (\ref{eq:md}) increases alignment scores for node pairs that have high \Quan{}.
%Indeed, the \Quan{} for all node pairs $(i, i')$ given the alignment matrix $\TB$, can be written as a matrix $\SB=[S_{ii'}]$ 
%	\begin{equation*}
%		\SB(\TB)=\exp\Big(2\BB^\src\TB\BB^\tar-h(\BB^\src)\pB\otimes\oneB-\oneB\otimes h(\BB^\tar)\qB\Big),
%	\end{equation*}
%such that $\ehdc(i,i';\TB)=S_{ii'}$.
%Therefore, iteration $\tau$ can also be written as $\TB^{(\tau+1)}=\proj_{\Pi^{|\VM^\src|}}\Big(\TB^{(\tau)}\odot\exp(-\JB)\odot\SB(\TB^{(\tau)})^{\eta^{(\tau)}}\Big)$, where the exponentiation is element-wise.

%Eq. (\ref{eq:mirror descent}) implies that each iteration (\ref{eq:md}) increases alignment scores for node pairs that have high \Quan{}.
%Indeed, we have the following proposition.
%\begin{proposition}\label{prop:matrix Quan}
%	The \Quan{} for all node pairs $(i, i')$ given the alignment matrix $\TB$, can be written as a matrix $\SB=[S_{ii'}]$ 
%	\begin{equation*}
%		\SB(\TB)=\exp\Big(2\BB^\src\TB\BB^\tar-h(\BB^\src)\pB\otimes\oneB-\oneB\otimes h(\BB^\tar)\qB\Big),
%	\end{equation*}
%	such that $\ehdc(i,i';\TB)=S_{ii'}$.
%\end{proposition}
%Therefore, iteration $\tau$ can also be written as $\TB^{(\tau+1)}=\proj_{\Pi^{|\VM^\src|}}\Big(\TB^{(\tau)}\odot\exp(-\JB)\odot\SB(\TB^{(\tau)})^{\eta^{(\tau)}}\Big)$, where the exponentiation is element-wise.

We demonstrate that low topology violation for matched node pairs is a necessary condition for accurate alignment.
%On the one hand, accurate alignment entails high \Quan{}.
In particular, if $\GM^\src$ is isomorphic to a subgraph of $\GM^\tar$ that is induced by the true counterpart nodes,
up to a few noisy or missing edges,
$d\big(i,\pi^*(i);\TB^*\big)$ values are low where $\pi^*:\VM^\src\to\VM^\tar$ and $\TB^*=[T_{ii'}^*]$ are the true matching and its matrix form, respectively.
This is formalized in the following theorem.
\begin{theorem}\label{thm:principle}
	Let $\DeltaB^{(k)}=[\Delta^{(k)}_{jj'}]\in\RBB^{|\VM^\src|\times|\VM^\tar|}$ denote the perturbation to the edge structure, which is given by $\DeltaB^{(k)}=(\LB^\src)^k-\TB^{*}(\LB^\tar)^k\TB^{*\top}$.
	Assume that for all $i$,
	the perturbation to the local topology is bounded by $\sum_{j\in\NM_k^\src(i),j'\in\NM_k^\tar(\pi^*(i'))}|\Delta^{(k)}_{jj'}|^2\le\epsilon^{(k)}$.
	Then $\maQuan\big(i,\pi^*(i);\TB^*\big)$ can be bounded from below as follows:
	\begin{equation*}
		d\big(i,\pi^*(i);\TB^*\big)\le K\sum_{k=1}^{K}\Big(\frac{(-t)^k}{k!}\Big)^2\epsilon^{(k)}.
	\end{equation*}
%	\begin{equation*}
%		\maQuan\big(i,\pi^*(i);\TB^*\big)\ge\exp\Big(-K\sum_{k=1}^{K}\Big(\frac{(-t)^k}{k!}\Big)^2\epsilon^{(k)}\Big).
%	\end{equation*}
\end{theorem}
%Theorem \ref{thm:principle} implies that $\maQuan\big(i,\pi^*(i);\TB^*\big)$ is close to $1$ for a small $s$.
%When $k$ is small, $\epsilon^{(k)}$ is small.
%As is required by heat diffusion wavelet, $s$ is usually small.
%Therefore, by choosing a small $s$, $\maQuan\big(i,\pi^*(i);\TB^*\big)$ is close to $1$.
The small-world property of real graphs suggests that a small $K$ is enough in practice \citep{watts1998collective}.
To capture local topology, $t$ is a small value \citep{tsitsulin2018netlsd,donnat2018learning}.
Therefore, $d\big(i,\pi^*(i);\TB^*\big)$ is close to 0.
%Therefore, $\maQuan\big(i,\pi^*(i);\TB^*\big)$ is close to $1$.

The mirror descent-based update allows $d\big(i,\pi^*(i);\TB^*\big)$ values for matched node pairs to decrease gradually,
which we formalize in the following theorem.
%The high-level idea is that when the topology violation for true node pairs is much lower than the topology violation
\begin{theorem}\label{thm:mirror descent assumptions}
	When we use \method{} to match graphs of the same number of nodes,
	if the following assumptions hold:
	\begin{enumerate}
		\item $\alpha^{(\tau)}\ge d(i,\hat{i};\TB^{(\tau)})$ for all $i$ where $\hat{i}=\argmax_{i'}T_{ii'}$,
		\item $\beta^{(\tau)}\le d(i,i';\TB^{(\tau)})$ for all $i$ where $i'\neq \hat{i}$,
		\item $|\VM^\src|\exp(\alpha^{(\tau)}\eta^{(\tau)})\le\exp(\beta^{(\tau)}\eta^{(\tau)})$ for all $i$,
	\end{enumerate}
	the topology violation values for all $(i,\hat{i})$ decrease at iteration $\tau$, $d(i,\hat{i};\TB^{(\tau+1)})\ge d(i,\hat{i};\TB^{(\tau)})$.
\end{theorem}
According to Proposition \ref{prop:relationship with MNC} and Theorem \ref{thm:mirror descent assumptions}, \method{} with $K=1$ and $t=1$ can also be viewed as maximizing a lower bound of $\operatorname{MNC}(i, i^*;\pi^*)$ for all true node pairs.


%We further note that the true matching matrix $\TB^*$ is a fixed point for the mirror descent-based optimization.
%\begin{theorem}\label{thm:fixed point}
%	$\TB^*$ is a fixed point for iteration (\ref{eq:md}).
%\end{theorem}


%To alleviate (near) structural indistinguishability,
%one may take a larger neighborhood into account.

%On the other hand, misalignment may occur but only for structurally indistinguishable nodes, as is shown in Theorem \ref{thm:indistinguishable}.
%
%\begin{theorem}\label{thm:indistinguishable}
%	If $\GM^\src$ is isomorphic to a subgraph of $\GM^\tar$, suppose that there exists $\pi(\cdot)$ that yields $\maQuan=1$ for all matched node pairs.
%	Then, if $\pi$ misaligns a node $i$ to a node $i'$ instead of the true counterpart $i^*$,
%	it is because $\NM_k^\tar(i')$ is isomorphic to $\NM_k^\tar(i^*)$.
%\end{theorem}

%When $K=1$, \Quan{} has a more intuitive interpretation, which needs the following definition.
%\begin{definition}[mapped neighborhood]
%	The mapped neighborhood of node $i\in\VM^\src$ is the set of nodes in $\GM^\tar$ onto which $\pi$ maps $i$'s neighbors, i.e., $\tilde{\NM}_k^\src(i;\pi)=\{j'\in\VM^\tar|\exists j\in\NM_k^\src(i) \st \pi(j)=j'\}$.
%\end{definition}

%\citeauthor{chen2020cone} \citeyear{chen2020cone} and \citeauthor{heimann2021refining} \citeyear{heimann2021refining} define the \emph{matched neighborhood consistency} (MNC) of node $i$ in $\GM^\src$ and node $i'$ in $\GM^\tar$ to be the Jaccard similarity of the sets $\tilde{\NM}_1^{\src}(i;\pi)$ and $\NM_{1}^\tar(i')$, i.e., $\operatorname{MNC}(i, i';\pi)=\frac{\left|\tilde{\NM}_1^{\src}(i;\pi) \cap \NM_{1}^\tar(i')\right|}{\left|\tilde{\NM}_1^{\src}(i;\pi) \cup \NM_{1}^\tar(i')\right|}$.
%When $K=1$ and two graphs of the same number of nodes are to be matched, \Quan{} can be reduced to a form similar to MNC, which is stated in the following proposition.



%We further reveal that RefiNA proposed by \citeauthor{heimann2021refining}\citeyear{heimann2021refining} essentially maximizes the edge correctness (EC),
%which is defined as the ratio of the number of edges conserved by $\pi$ to the
%number of edges in the source network
%\citep{patro2012global},
%%\citep{patro2012global,saraph2014magna,sun2015simultaneous,mamano2017sana,xu2019scalable},
%\begin{equation*}
%	\maEC(\pi)=\frac{|\pi(\EM^\src)|}{|\EM^\src|}, \where \pi(\EM^\src)=\{\big(\pi(i),\pi(j)\big)\in\EM^\tar|\forall (i,j)\in\EM^\src\}.
%\end{equation*}
%RefiNA iteratively increases alignment scores for nodes that have high relaxed numerator values of MNC.
%Representing $\pi$ with the matrix form $\TB$ and relaxing the binary matching matrix to $\PM^f$,
%the gradient of $\maEC$ with respect to $\TB$ is $\WB^\src\TB\WB^\tar$, the relaxed numerator values of MNC values \citep{heimann2021refining}.
%As is shown in \citet{saraph2014magna}, EC does not penalize alignments mapping sparser network regions to denser ones, which negatively affects the alignment accuracy and leaves room for improvement.


















==> local_topology arxiv/sections/new_method.tex <==
%Leveraging the insights from the theory in Sec. \ref{sec:si}, we propose an unsupervised graph matching algorithm named \method{}.
%We also discuss its relationship to state-of-the-art methods.

%\subsection{Algorithm}

We update the matching matrix based on the \sis{} matrix.
The high level intuition is that each iteration decreases alignment scores for node pairs that have relatively high \sis{} values.
The recurrence of \method{} reads
\begin{equation}\label{eq:iteration}
	\TB^{(\tau+1)}=\proj_{\CM}\TB^{(\tau)}\odot\exp\big(-\eta^{(\tau)}\SB(\TB^{(\tau)})\big),
\end{equation}
where $\tau=0,1,\dots$, $\odot$ is the element-wise multiplication and the exponentiation is also element-wise.
The projection can be solved via Sinkhorn-Knopp algorithm with linear convergence rate \citep{sinkhorn1967concerning}.

Actually, iteration (\ref{eq:iteration}) is the mirror descent update for calculating the GW distance.
To solve problem
\begin{equation}\label{eq:real objective}
	\min_{\TB\in\Pi(\oneB, \oneB)}f(\TB):=\sum_{i=1}^{|\VM^\src|}\sum_{j=1}^{|\VM^\src|}\sum_{i'=1}^{|\VM^\tar|}\sum_{j'=1}^{|\VM^\tar|}(B_{ij}^\src-B_{i'j'}^\tar)^2T_{ii'}T_{jj'},
\end{equation}
the most common algorithm is gradient descent that iteratively updates $\TB$ as follows
\begin{equation}\label{eq:gd}
	\TB^{(\tau+1)}=\proj_{\Pi(\oneB, \oneB)}\Big\{\TB^{(\tau)}-\eta^{(\tau)}\nabla f(\TB^{(\tau)})\Big\},
\end{equation}
where the gradient reads
\begin{equation}\label{eq:gradient Ours}
	\nabla f(\TB)=h(\BB^\src)\oneB\otimes\muB^\src+\oneB\otimes h(\BB^\tar)\muB^\tar-2\BB^\src\TB\BB^\tar,
\end{equation}
Mirror descent takes into account the geometry of the feasible domain \citep{bubeck2015convex}, and is better-suited to Problem (\ref{eq:real objective}).
Mirror descent is given by the recurrence
\begin{equation}\label{eq:md 0}
	\TB^{(\tau+1)}=\argmin_{\TB\in\Pi(\oneB, \oneB)}\langle \nabla f(\TB^{(\tau)}),\TB\rangle+\frac{1}{\eta^{(\tau)}}D_\psi(\TB,\TB^{(\tau)}),
\end{equation}
where $D_\psi(\TB,\TB^{(\tau)})$ stands for the Bregman divergence.
%where $D_\psi(\TB,\TB^{(\tau)})=\psi(\TB)-\psi(\TB^{(\tau)})-\langle\nabla\psi(\TB^{(\tau)}),\TB-\TB^{(\tau)}\rangle$ stands for the Bregman divergence generated by a strongly convex and continuously differentiable function $\psi(\TB)$.
When one selects the generalized KL-divergence $\KL(\AB|\BB)=\sum_{ij}A_{ij}\log\frac{A_{ij}}{B_{ij}}-A_{ij}+B_{ij}$ as the Bregman divergence,
(\ref{eq:md 0}) becomes iteration (\ref{eq:iteration}).


\begin{algorithm}[ht]
	\caption{\method{} \label{alg:method}}
	\begin{algorithmic}[1]
		\State {\textbf{Input:}} Total rounds $T$, graphs $\GM^\src$ and $\GM^\tar$, initial transport plan $\TB^{(0)}$.
		\State {\textbf{Output:}} Correspondence set $\CM$.
		\State Calculate and store matrices $\BB^\src$ and $\BB^\tar$.
		\For{$\tau=0,\dots,T-1$}
		\State Update $\TB^{(\tau+1)}$ by iteration \ref{eq:iteration}.
		\EndFor
		\State $\tilde{\TB}=\TB^{(T)}$
		\State Initialize correspondence set $\CM=\emptyset$
		\For{$i\in\VM^\src$}
		\State $i'=\arg\max_{i'} \tilde{T}_{ii'}$.
		\State $\CM=\CM\cup\{(i,i')\}$
		\EndFor
	\end{algorithmic}
\end{algorithm}

\method{} is summarized in Algorithm \ref{alg:method}.
The matching cost is based on heat diffusion wavelets.
It updates the matching matrix using (\ref{eq:iteration}).
By choosing the largest index from $\tilde{\TB}[i,:]$ for each $i$, we find the correspondence.




==> local_topology arxiv/sections/preliminary.tex <==
In this section, we give basic preliminary to facilitate the later discussion and review the main background.

Here, we first give the notations used in the main text. 
We use bold lowercase symbols, bold uppercase letters, and uppercase calligraphic fonts to denote vectors (e.g. $\xB$), matrices (e.g. $\AB$), and sets (e.g. $\AM$), respectively.
$(\cdot)^\top$ is the transpose of a vector or a matrix.
$\AB[i,:]$ and $\AB[:,j]$ are the $i$-th row and the $j$-th column of matrix $\AB$ respectively.
For two matrices $\AB$ and $\BB$ that are of the same size, $\langle \AB,\BB\rangle=\trace(\AB^\top\BB)$ is the Frobenius dot-product.
We denote the cardinality of set $\AM$ by $|\AM|$. 

%We use bold lowercase symbols, bold uppercase letters, uppercase calligraphic fonts, and Greek letters to denote vectors, matrices, spaces (sets), and measures, respectively.
%For example, $\alpha=\sum_i \delta_{\xB_i}(\xB)$ where $\delta_{\xB_i}(\xB)$ is the Dirac function at position $\xB_i$, is a discrete measure supported on $\xB_1,\dots,\xB_n\in \XM$.
%$(\cdot)^\top$ is the transpose of a vector or a matrix.
%$\AB[i,:]$ and $\AB[:,j]$ are the $i$-th row and the $j$-th column of matrix $\AB$ respectively.
%For two matrices $\AB$ and $\BB$ that are of the same size, $\langle \AB,\BB\rangle=\trace(\AB^\top\BB)$ is the Frobenius dot-product.
%We denote the cardinality of set $\AM$ by $|\AM|$. 
%%$\pi(\alpha,\beta)$ is a coupling measure between measures $\alpha$ and $\beta$, that is, for any subset $\AM\subset \XM$, $\pi(\AM\times\YM)=\alpha(\AM)$, and for any $\BM\subset\YM$, $\pi(\XM\times\BM)=\beta(\BM)$.
%%$\Pi(\alpha,\beta)$ denotes the set of coupling measures.
%$\Sigma^n$ is a probability symplex with $n$ bins, namely the set of probability vectors in $\RBB^n_{+}$.

\subsection{Graph Matching}
We consider undirected graphs without self-loops $\GM=(\VM,\EM,\WB)$, where $\VM$ is the set of vertices, $\EM$ is the set of edges, and  $\WB=[W_{ij}]\in\RBB^{|\VM|\times|\VM|}$ is a (binary or weighted) adjacency matrix.
If there is an edge $(i, j)$ connecting vertices $i$ and $j$, i.e., $(i,j)\in\EM$, the entry $W_{ij}$ represents the weight of the edge;
Otherwise, $W_{ij}=0$.
The degree of each vertex $i$, written as $d_i$, is defined as the sum of the weights of all the edges incident to it, i.e., $d_i=\sum_{j=1}^{|\VM|} W_{ij}$.
The degree matrix $\DB=[D_{ij}]$ has diagonal elements equal to the degrees $D_{ii}=d_i$, and zeros elsewhere.
The Laplacian matrix of $\GM$ is defined as $\LB=\DB-\WB$.
The $k$-hop neighborhood of node $i$, denoted by $\NM_k(i)$, is the subgraph of $\GM$ induced by all nodes that are $k$ or fewer hops away from node $i$.

Given the source graph $\GM^\src=(\VM^\src,\EM^\src,\WB^\src)$ and the target graph $\GM^\tar=(\VM^\tar,\EM^\tar,\WB^\tar)$,
assuming $|\VM^\src|\le|\VM^\tar|$ without loss of generality
graph matching aims to find an injective mapping $\pi:\VM^\src\to\VM^\tar$ that matches nodes in $\GM^\src$ to nodes in $\GM^\tar$.
In this paper, we focus on equal-size graph matching, i.e., $V=|\VM^\src|=|\VM^\tar|$.
In such case, $\pi$ is restricted to be a bijective.
For graphs with different number of nodes, one can add dummy isolated nodes into the smaller graph and make them equal-sized \citep{gold1996graduated,zaslavskiy2008path,jiang2017graph}.
$\pi$ is also commonly represented as a matching matrix $\TB\in\Big\{\TB\in\{0,1\}^{|\VM^\src|\times |\VM^\tar|}|\TB\oneB=\oneB,\TB^\top\oneB=\oneB\Big\}$ (eg. \citep{fey2019deep,heimann2021refining}),
where
\begin{equation}\label{eq:matching matrix}
	T_{ii'}=\begin{cases}
		1,& \text{ if } i \in\VM^\src \text{ is matched to } i'\in\VM^\tar,\\
		0,& \text{ else.}
	\end{cases}
\end{equation}

%\subsection{Heat Diffusion}
%Following the literature (e.g., \citep{shuman2013emerging,vijayan2015magna++,heimann2018regal,heimann2021refining}),
%we consider undirected graphs without self-loops, denoted as tuples of the form $\GM=(\VM,\EM,\WB)$ which consists of a finite set of vertices $\VM$, a set of edges $\EM$, and a (binary or weighted) adjacency matrix $\WB=[W_{ij}]\in\RBB^{|\VM|\times|\VM|}$.
%If there is an edge $(i, j)$ connecting vertices $i$ and $j$, i.e., $(i,j)\in\EM$, the entry $W_{ij}$ represents the weight of the edge;
%Otherwise, $W_{ij}=0$.
%The degree of each vertex $i$, written as $d_i$, is defined as the sum of the weights of all the edges incident to it, i.e., $d_i=\sum_{j=1}^{|\VM|} W_{ij}$.
%The degree matrix $\DB=[D_{ij}]$ has diagonal elements equal to the degrees $D_{ii}=d_i$, and zeros elsewhere.
%The Laplacian matrix of $\GM$ is defined as $\LB=\DB-\WB$.
%
%%Recently, there has been significant interest in designing \emph{heat diffusion}-based methods to capture the structural information of graphs (eg. \citep{tsitsulin2018netlsd,berberidis2018adaptive,donnat2018learning,klicpera2019diffusion}).
%The heat diffusion on a graph is the solution to the discrete heat equation \citep{kondor2002diffusion}.
%%To describe the diffusion process on $\GM$,
%%Let $\vB(t)\in\RBB^{|\VM|}$ be a time-varying vector that represents the diffusion process on the graph.
%Particularly, let $\vB(t)\in\RBB^{|\VM|}$ represent the heat of each vertex at time $t$.
%The edge weight $W_{ij}$ describes the conductivity between vertices,
%so that for two vertices $i$ and $j$,
%the quantity $W_{ij}\big(v_i(t)-v_j(t)\big)$ represents the flux from vertex $i$ to vertex $j$.
%Summing over these fluxes for each vertex yields $v'_j(t)=\sum_i W_{ij}\big(v_i(t)-v_j(t)\big)$.
%It can be verified that
%\begin{equation}\label{eq:derivative heat diffusion}
%	\vB'(t)=-\LB\vB(t).
%\end{equation}
%Equation (\ref{eq:derivative heat diffusion}) has the analytic solution $\vB(t)=\exp(-t\LB)\vB(0)$.
%Here $\exp(-t\LB)=\sum_{k=0}^{\infty}\frac{(-t)^k}{k!}\LB^k$ is a $|\VM|\times|\VM|$ matrix-valued fuction of $t$, known as the Laplacian exponential diffusion kernel \citep{hammond2013graph}.
%As $t$ approaches zero,
%high-order terms vanish,
%meaning that the kernel depicts \emph{local connectivity} \citep{tsitsulin2018netlsd,donnat2018learning}.
%Intuitively, each node propagates a unit of energy over the graph and the local topology is characterized by the amount of energy that each neighboring node receives after a given time.
%It can be proved that nodes that share similar local topology have similar diffusion patterns \citep{donnat2018learning}.
%
%Therefore, heat diffusion allows us to characterize the multi-hop neighborhood of each node and match node pairs that have similar local topological structures.
%%The heat diffusion provides a way to quantify the network connectivity between a pair of nodes and characterize the local topology \citep{donnat2018learning,klicpera2019diffusion}.
%The $K$-th order approximation of $\exp(-t\LB)$ is
%\begin{equation}\label{eq:heat diffusion wavelet}
%	\PsiB=\sum_{k=0}^{K}\frac{(-t)^k}{k!}\LB^k.
%\end{equation}
%The $i$-th row, $\PsiB[i,:]$, is the $K$-th order \emph{heat diffusion wavelet} for node $i$ \citep{donnat2018learning}.
%%$\PsiB$ is localized in the $K$-hop neighborhood of a node $i$,
%%i.e.,
%%$\Psi_{ij}=0$ if nodes $i$ and $j$ are not connected with a path of less than or equal to $K$ hops on the graph.
%%Entry $\Psi_{ij}$ contains
%%%terms of the form $\DB^k$ 
%%terms of the form $\WB^K$ (the sum of the products of all weights of all paths from node $i$ to every other node $j$ of length exactly $K$), and terms containing both $\DB$ and $\WB$, which denote paths of length up to $K$ going from $i$ to $j$.
%$\PsiB[i,:]$ measures the network connectivity between node $i$ and each node $j$.
%%and characterizes the local topological structure of node $i$.
%
%%\subsection{Random Walk}
%%Another way ...

\subsection{Optimal Transport}
Given two discrete measures $\alpha=\sum_{i=1}^{m}p_i\delta_{\xB_i}(\xB)$ and $\beta=\sum_{j=1}^{n}q_j\delta_{\yB_j}(\yB)$,
Optimal transport (OT) addresses the problem of optimally transporting $\pB=[p_i]\in\RBB_+^m$ toward $\qB=[q_j]\in\RBB_+^n$ \citep{villani2008optimal}.
The $p$-Wasserstein distance between $\pB$ and $\qB$ is defined as
\begin{equation*}
	W_p^p(\pB,\qB)=\min_{\TB\in\Pi(\pB,\qB)}\langle \KB^p,\TB \rangle,
\end{equation*}
where $K_{ij}$ is the distance between $\xB_i$ and $\yB_j$, $\KB^p=[K_{ij}^p]\in\RBB_+^{m\times n}$ and the feasible domain of \emph{transport plan} $\TB$ is given by the set of \emph{coupling measures} $\Pi(\pB,\qB)=\{\TB\in\RBB_+^{m\times n}|\TB\oneB_n=\pB,\TB^\top\oneB_m=\qB\}$.

Gromov-Wasserstein (GW) distance is a generalization of Wasserstein distance \citep{memoli2011gromov}.
Let $\XM$ and $\YM$ be two sample spaces.
Endowing the spaces $\XM$ and $\YM$ with metrics (distances) $d_\XM$ and $d_\YM$,
the GW distance is defined as
\begin{equation*}
	GW_p^p(\pB,\qB)=\min_{\TB\in\Pi(\pB,\qB)}\sum_{i,j=1}^{m}\sum_{i',j'=1}^{n}D_{ii'jj'}^pT_{ii'}T_{jj'},
\end{equation*}
where $D_{ii'jj'}=|d_\XM(\xB_i,\xB_j)-d_\YM(\yB_{i'},\yB_{j'})|$  with $\xB_1,\dots,\xB_m\in\XM$ and $\yB_1,\dots,\yB_n\in\YM$.

Optimal transport can be applied to graph matching.
The source graph $\GM^\src$ and the target graph $\GM^\tar$ are modelled as two probability distributions $\muB^\src=[\mu^\src_i]$ and $\muB^\tar=[\mu^\tar_i]$ respectively,
where
\begin{equation*}
	\mu^z_i=\frac{\sum_{j=1}^{|\VM^z|} W_{ij}^z}{\sum_{i=1}^{|\VM^z|}\sum_{j=1}^{|\VM^z|}W_{ij}^z}, \text{ for }z=\src,\tar.
\end{equation*}
A dissimilarity matrix $\BB^\src$ can be assigned to $\GM^\src$ to encode the structural information.
Each entry $B_{ij}^\src$ models the distance between nodes $i$ and $j$ in $\GM^\src$,
such as the edge weight-based distance \citep{xu2019gromov}, the shortest path distance, or the harmonic distance \citep{verma2017hunt}.
$\BB^\tar$ is defined similarly.
Basically, the node correspondence is estimated by calculating the transport plan of the Gromov-Wasserstein distance that is defined as $GW(\muB^\src,\muB^\tar)=\min_{\TB\in\Pi(\muB^\src,\muB^\tar)}\ell(\TB)$, where
\begin{equation}\label{eq:Xu GW}
	\ell(\TB)=\sum_{i=1}^{|\VM^\src|}\sum_{j=1}^{|\VM^\src|}\sum_{i'=1}^{|\VM^\tar|}\sum_{j'=1}^{|\VM^\tar|}(B_{ij}^\src-B_{i'j'}^\tar)^2T_{ii'}T_{jj'}.
\end{equation}
Node $i\in\VM^\src$ is matched to $\hat{i}\in\VM^\tar$,
where $\hat{i}=\argmax_{i'}T^*_{ii'}$ and $\TB^*$ attains the minimum of Eq. (\ref{eq:Xu GW}).

Note that to better approximate matching matrices (\ref{eq:matching matrix}),
one can relax the feasible domain from $\Big\{\TB\in\{0,1\}^{V\times V}|\TB\oneB=\oneB,\TB^\top\oneB=\oneB\Big\}$ to $\Pi(\oneB,\oneB)=\Big\{\TB\in[0,1]^{V\times V}|\TB\oneB=\oneB,\TB^\top\oneB=\oneB\Big\}$,
instead of $\TB\in\Pi(\muB^\src,\muB^\tar)$.
The matching matrix can then be interpreted as a transport plan from $\oneB$ to $\oneB$.

%The Wasserstein distance and the GW distance require the two marginals to have the same total mass
%$\|\pB\|_1 = \|\qB\|_1$ and that all the mass has to be transported.
%The partial OT problem focuses on transporting only a fraction $0\le b\le \min\{\|\pB\|_1, \|\qB\|_1\}$ of the mass with minimum transportation costs \citep{figalli2010optimal,caffarelli2010free,chapel2020partial}, that is, the set of admissible couplings is given by
%\begin{equation*}
%	\Pi^b(\pB,\qB)=\Big\{\TB\Big|\TB\in\RBB_+^{m\times n},\TB\oneB\le\pB,\TB^\top\oneB\le\qB,\oneB^\top\TB\oneB=b\Big\}.
%\end{equation*}
%The partial GW distance is defined as
%\begin{equation*}
%	\begin{aligned}
%		PGW_p^p(\pB,\qB)&=\min_{\TB\in\Pi^b(\pB,\qB)}\sum_{i,j=1}^{m}\sum_{i',j'=1}^{n}D_{ii'jj'}^pT_{ii'}T_{jj'}.
%	\end{aligned}
%\end{equation*}
%The partial Wasserstein distance and the partial GW distance are defined respectively as follows
%\begin{equation*}
%	\begin{aligned}
%		PW_p^p(\pB,\qB)&=\min_{\TB\in\Pi^b(\pB,\qB)}\langle \KB^p,\TB \rangle,\\
%		PGW_p^p(\pB,\qB)&=\min_{\TB\in\Pi^b(\pB,\qB)}\sum_{i,j=1}^{m}\sum_{i',j'=1}^{n}D_{ii'jj'}^pT_{ii'}T_{jj'}.
%	\end{aligned}
%\end{equation*}
%For graphs with different sizes, partial GW distance can be applied to graph matching, as we shall see in Sec. \ref{sec:method}.

\subsection{Heat Diffusion Wavelet}

For each graph $z=\src,\tar$,
the heat diffusion on a graph is the solution to the discrete heat equation,
$\vB(t)=\exp(-t\LB^z)\vB(0)$ where $\vB(t)\in\RBB^{|\VM^z|}$ represent the heat of each vertex at time $t$ and $\exp(-t\LB^z)=\sum_{k=0}^{\infty}\frac{(-t)^k}{k!}(\LB^z)^k$ \citep{kondor2002diffusion}.
$\exp(-t\LB)=\sum_{k=0}^{\infty}\frac{(-t)^k}{k!}\LB^k$ is a $|\VM|\times|\VM|$ matrix-valued fuction of $t$, known as the Laplacian exponential diffusion kernel \citep{hammond2013graph}.
As $t$ approaches zero,
high-order terms vanish,
meaning that the kernel depicts \emph{local connectivity} \citep{tsitsulin2018netlsd,donnat2018learning}.
The $K$-th order approximation of $\exp(-t\LB^z)$ is
\begin{equation}\label{eq:heat diffusion wavelet}
	\PsiB=\sum_{k=0}^{K}\frac{(-t)^k}{k!}(\LB^z)^k.
\end{equation}
The $i$-th row, $\PsiB[i,:]$, is the $K$-th order HDW for node $i$ \citep{donnat2018learning} and measures the network connectivity between node $i$ and each node $j$.
%It can be proved that nodes that share similar local topology have similar heat diffusion wavelets \citep{donnat2018learning}.
$\BB^z=[B_{ij}^z]$ that characterizes node dissimilarities within each graph is defined as
\begin{equation}
	B_{ij}^z=\begin{cases}
		&\bar{\Psi}-\Psi_{ij}^z,\text{ if }i\neq j,\\
		&0, \text{ else,}
	\end{cases}
\end{equation}
where $\Psi_{ij}^z$ is defined as Eq. (\ref{eq:heat diffusion wavelet}), $z=\src,\tar$ and constant $\bar{\Psi}>\max_{i,j,z}\Psi_{ij}^z$.




==> local_topology arxiv/sections/proof.tex <==

\subsection{Missing Proofs of Sec. \ref{sec:si}}

%\paragraph{Proof of Proposition\ref{prop:transport distance}.}
%
%Since $\GM^\src$ and $\GM^\tar$ are isomorphic, $\mu_i^\src=\mu_{i^*}^\tar$ for all \groundtruth{} node pairs $(i,i^*)$.
%By setting $C_{ij}^z=\frac{1}{1+W_{ij}^z}$ for $z=\src,\tar$, we have $C_{ij}^\src=C_{i'j'}^\tar$ when $i'=i^*$ and $j'=j^*$.
%Because $(C_{ij}^\src-C_{i'j'}^\tar)^2\ge0$, $GW(\muB^\src,\muB^\tar)\ge0$.
%
%Define $\tilde{\TB}=[\tilde{T}_{ii'}]$ such that $\tilde{T}_{ii'}=\mu_i^\src$ if $i'=i^*$ and $\tilde{T}_{ii'}=0$ otherwise.
%It can be verified that $\tilde{\TB}\in\Pi(\muB^\src,\muB^\tar)$.
%For each item $(C_{ij}^\src-C_{i'j'}^\tar)^2\tilde{T}_{ii'}\tilde{T}_{jj'}$,
%either $\tilde{T}_{ii'}=0$ (resp. $\tilde{T}_{jj'}=0$) when $i'\neq\i^*$ (resp. $j'\neq j^*$),
%or $C_{ij}^\src=C_{i'j'}^\tar$ when $i'=i^*$ and $j'=j^*$.
%Therefore, the objective reaches minimum 0, which implies $\TB^*=\tilde{\TB}$.
%
%For $G_{ii^*}(\TB^*)$, we have
%\begin{equation*}
%	G_{ii^*}(\TB^*)=\sum_{j=1}^{|\VM^\tar|}\sum_{j'=1}^{|\VM^\tar|}T_{jj'}(C_{ij}^\src-C_{i^*j'}^\tar)^2=\sum_{j=1}^{|\VM^\tar|}T_{jj^*}(C_{ij}^\src-C_{i^*j^*}^\tar)^2=0.
%\end{equation*}
%
%For $G_{ii'}(\TB^*)$, we have
%\begin{equation*}
%	G_{ii'}(\TB^*)=\sum_{j=1}^{|\VM^\tar|}T_{jj^*}(C_{ij}^\src-C_{i'j^*}^\tar)^2.
%\end{equation*}
%\begin{flushright}
%	$\blacksquare$
%\end{flushright}

\paragraph{Proof of Theorem \ref{thm:indistinguishable}.}

Since graph isomorphism is transitive, it suffices to prove that $\NM_K^\src(i)$ is isomorphic to $\NM_K^\tar(\hat{i})$, which we prove by contradiction.
Denote the matching induced by $\TB$ as $\pi:\VM^\src\to\VM^\tar$, i.e., $\pi(i)=\argmax_{i'}T_{ii'}$.
Suppose $\NM_K^\src(i)$ is not isomorphic to $\NM_K^\tar(\hat{i})$.
Then there exists neighboring nodes $a,b\in\NM_K^\src(i)$ where either $\pi(a)$ or $\pi(b)$ is not in $\NM_K^\tar(\hat{i})$, or $\pi(a)$ and $\pi(b)$ do not share an edge.

In case 1, without loss of generality, $\pi(b)\notin\NM_K^\tar(\hat{i})$.
Then $\masis(i,\hat{i};\TB)\ge T_{b\pi(b)}(B_{ib}^\src-B_{\hat{i}\pi(b)}^\tar)^2>0$: a contradiction.

In case 2, since $\pi(b)$ is the counterpart of a neighbor of $a$, it must also be a neighbor of the counterpart of $a$ which is a contradition of the assumption that $\pi(a)$ and $\pi(b)$ do not share an edge,
or else $\masis\big(a,\pi(a)\big)>0$, another contradiction.

Therefore, we conclude that $\NM_K^\src(i)$ and $\NM_K^\tar(\hat{i})$ are isomorphic.

\begin{flushright}
	$\blacksquare$
\end{flushright}

\paragraph{Proof of Theorem \ref{thm:principle}.}


%We bound $\maQuan(i,\pi^*(i);\TB^*)$ from below by bounding $d(i,\pi^*(i);\TB^*)$ from above.

For \groundtruth{} node pairs $(i,i^*)$ and \groundtruth{} matching matrix, denoting $a_k=\frac{(-t)^k}{k!}$, we have
\begin{equation*}
	\begin{aligned}
		\masis(i,i^*;\TB^*)&=\sum_{j=1}^{|\VM^\tar|}(B_{ij}^\src-B_{i^*j^*}^\tar)^2\\
		&\overset{\textcircled{1}}{=}\sum_{j=1}^{|\VM^\tar|}\Big(\sum_{k=1}^{K}a_k[(\LB^\src)^k]_{ij}-a_k[\TB^*(\LB^\tar)^k\TB^{*\top}]_{ij}\Big)^2\\
		&\overset{\textcircled{2}}{\le}\sum_{j=1}^{|\VM^\tar|}K\sum_{k=1}^{K}(a_k)^2\Big([(\LB^\src)^k]_{ij}-[\TB^*(\LB^\tar)^k\TB^{*\top}]_{ij}\Big)^2\\
		&\overset{\textcircled{3}}{\le}K\sum_{k=1}^{K}(a_k)^2\epsilon_k,
	\end{aligned}
\end{equation*}
where we substitute the definitions of $B_{ij}^\src$ and $B_{i^*j^*}^\tar$ into equality \textcircled{1},
use the Cauchy–Schwarz inequality in inequality \textcircled{2},
and use the definition of $\epsilon_k$ in inequality \textcircled{3}.
\begin{flushright}
	$\blacksquare$
\end{flushright}



\subsection{Missing Proofs of Sec. \ref{sec:theory}}

\paragraph{Proof of Lemma \ref{lem:mirror descent assumptions}.}


%The mirror descent recurrence is $\TB^{(\tau+1)}=\proj_{\Pi^{|\VM^\src|}}\Big(\frac{1}{e}\TB^{(\tau)}\odot \eta^{(\tau)}\GB(\TB)\Big)$.
%To match graphs of the same number of nodes,
%the projection is identical to Sinkhorn scaling \citep{knight2008sinkhorn},
%that is,
%\begin{equation*}
%	\TB^{(\tau+1)}=\Diag(\uB)\YB\Diag(\vB),
%\end{equation*}
%where $\YB=\frac{1}{e}\TB^{(\tau)}\odot \eta^{(\tau)}\GB(\TB)$, and $\uB=[u_i],\vB=[v_{i'}]\in\RBB_+^{|\VM^\src|}$.
The mirror descent recurrence is $\TB^{(\tau+1)}=\proj_{\Pi(\oneB,\oneB)}\Big(\TB^{(\tau)}\odot \GB(\TB^{(\tau)})\Big)$,
where $\GB(\TB^{(\tau)})=\exp\Big(-\eta^{(\tau)}h(\BB^\src)\oneB\otimes\oneB-\eta^{(\tau)}\oneB\otimes h(\BB^\tar)\oneB+2\eta^{(\tau)}\BB^\src\TB^{(\tau)}\BB^\tar\Big)$.
The projection is achieved by Sinkhorn scaling \citep{knight2008sinkhorn},
that is,
\begin{equation*}
	\TB^{(\tau+1)}=\Diag(\uB)\YB\Diag(\vB),
\end{equation*}
where $\YB=\TB^{(\tau)}\odot \GB(\TB^{(\tau)})$, and $\uB,\vB\in\RBB_+^{V}$.

The recurrence implies that,
\begin{equation}\label{eq:beta}
	Y_{ii'}= T_{ii'}^{(\tau)}\exp\big(-\eta^{(\tau)}\masis(i,i';\TB^{(\tau)})\big).
\end{equation}

The feasible domain requires that
\begin{equation*}
	1=\sum_{i'}u_iY_{ii'}v_{i'}, \text{ and }1=\sum_{i}u_iY_{ii'}v_{i'}.
\end{equation*}
Hence,
\begin{equation}\label{eq:alpha}
	v_{i'}=\frac{1}{\sum_{i}u_iY_{ii'}}\le\frac{1}{u_iY_{ii^*}}= \frac{1}{u_iT_{ii^*}^{(\tau)}\exp\Big(-\eta^{(\tau)}\macsi(i;\TB^{(\tau)})\Big)},
\end{equation}
where the first inequality is due to the fact that $u_i\ge0$ and $Y_{ii'}\ge0$.

Combining Eq. (\ref{eq:alpha}), (\ref{eq:beta}), and $\frac{1}{T_{ii^*}^{(\tau)}}\exp\Big(\eta^{(\tau)}\macsi(i;\TB^{(\tau)})\Big)\le\exp\Big(\eta^{(\tau)}\masis(i;i';\TB^{(\tau)})\Big)$,
we have $T_{ii'}^{(\tau+1)}\le T_{ii'}^{(\tau)}$ for $i'\neq i^*$.

%Using Theorem \ref{thm:each step}, we have $\maQuan(i,\hat{i};\TB^{(\tau+1)})\ge\maQuan(i,\hat{i};\TB^{(\tau)})$.

\begin{flushright}
	$\blacksquare$
\end{flushright}

\paragraph{Proof of Theorem \ref{thm:each step}.}

By the definition of the \si{},
\begin{equation*}
	\begin{aligned}
		\masis(i,i^*;\TB)&=\sum_{j\in\NM_K^\src(i)}T_{jj^*}(B_{ij}^\src-B_{i^*j^*}^\tar)^2+\sum_{j\notin\NM_K^\src(i)}T_{jj^*}(B_{ij}^\src-B_{i^*j^*}^\tar)^2+\sum_{j=1}^{|\VM^\src|}\sum_{j'\neq j^*}T_{jj'}(B_{ij}^\src-B_{i^*j'}^\tar)^2\\
		&=\sum_{j=1}^{|\VM^\src|}\sum_{j'\neq j^*}T_{jj'}(B_{ij}^\src-B_{i^*j'}^\tar)^2.
	\end{aligned}
\end{equation*}
Where the second equality is due to the fact that $\NM_K^\src(i)$ is isomorphic to $\NM_K^\tar(i^*)$ and $B_{ij}^\src=B_{i^*j^*}^\tar=\bar{\Psi}$ if node $j$ is more than $K$ hops away from node $i$.
If $T_{ii'}^{(\tau+1)}\le T_{ii'}^{(\tau)}$ for all $i$ and $i'\neq i^*$,
\begin{equation*}
	\masis(i,i^*;\TB^{(\tau+1)})=\sum_{j=1}^{|\VM^\src|}\sum_{j'\neq j^*}T_{jj'}^{(\tau+1)}(B_{ij}^\src-B_{i'j^*}^\tar)^2\le \sum_{j=1}^{|\VM^\src|}\sum_{j'\neq j^*}T_{jj'}^{(\tau)}(B_{ij}^\src-B_{i'j^*}^\tar)^2.
\end{equation*}
The right hand side of the inequality is exactly $\masis(i,i^*;\TB^{(\tau)})$.

%By the definition of the transport distance,
%\begin{equation*}
%	\begin{aligned}
%		G_{i\hat{i}}(\TB)&=\sum_{j\in\NM_k^\src(i)}T_{j\hat{j}}(C_{ij}^\src-C_{\hat{i}\hat{j}}^\tar)^2+\sum_{j\notin\NM_k^\src(i)}T_{j\hat{j}}(C_{ij}^\src-C_{\hat{i}\hat{j}}^\tar)^2+\sum_{j=1}^{|\VM^\src|}\sum_{j'\neq \hat{j}}T_{jj'}(C_{ij}^\src-C_{\hat{i}j'}^\tar)^2\\
%		&=\sum_{j=1}^{|\VM^\src|}\sum_{j'\neq \hat{j}}T_{jj'}(C_{ij}^\src-C_{\hat{i}j'}^\tar)^2.
%	\end{aligned}
%\end{equation*}
%Where the second equality is due to the fact that $\NM_k^\src(i)$ is isomorphic to $\NM_k^\tar(\hat{i})$ and $C_{ij}^\src=C_{\hat{i}\hat{j}}^\tar=\bar{\Psi}$ if node $j$ is more than $k$ hops away from node $i$.
%If $T_{ii'}^{(\tau+1)}\le T_{ii'}^{(\tau)}$ for all $i$ and $i'\neq \hat{i}$,
%\begin{equation*}
%	G_{i\hat{i}}(\TB^{(\tau+1)})=\sum_{j=1}^{|\VM^\src|}\sum_{j'\neq \hat{j}}T_{jj'}^{(\tau+1)}(C_{ij}^\src-C_{i'\hat{j}}^\tar)^2\le \sum_{j=1}^{|\VM^\src|}\sum_{j'\neq \hat{j}}T_{jj'}^{(\tau)}(C_{ij}^\src-C_{i'\hat{j}}^\tar)^2.
%\end{equation*}
%The right hand side of the inequality is exactly $G_{i\hat{i}}(\TB^{(\tau)})$.

\begin{flushright}
	$\blacksquare$
\end{flushright}





%\paragraph{Proof of Theorem \ref{thm:fixed point}.}
%
%It is easy to verify that the \groundtruth{} matching matrix $\TB^*$ belongs to the feasible domain, $\TB^*\in\Pi^{|\VM^\src|}$.
%In particular, each row has exactly one non-zero entry $T^*_{ii^*}=1$.
%Each column has no or one non-zero entry because $|\VM^\src|\le|\VM^\tar|$.
%
%The mirror descent update can be written as $\proj_{\Pi^{|\VM^\src|}}(\YB)$, where $\YB=\frac{1}{e}\TB^{*}\odot\SB(\TB^*)^{\eta}$ and $\odot$ denotes the element-wise multiplication.
%Both calculating $\YB$ and periodic projections can be considered as multiplying different scalars to $\TB^*$.
%After project ing back to the feasible domain $\Pi^{|\VM^\src|}$,
%non-zero entries become 1,
%that is,
%$\TB^*=\proj_{\Pi^{|\VM^\src|}}(\YB)$.
%
%\begin{flushright}
%	$\blacksquare$
%\end{flushright}

\paragraph{Proof of Theorem \ref{thm:md}}
We can rewrite the transport plan $\TB$ as a vector variable $\xB\in\RBB_+^{V^2}$ and the Gromov-Wasserstein distance Eq. (\ref{eq:real objective}) as objective $f(\xB)=\xB^\top\AB\xB$, respectively.

It is easy to verify that
\begin{enumerate}
	\item The feasible domain is a closed convex set.
	\item $f(\xB)$ is a weakly convex function.
	\item The norm of the gradient $\|\nabla f(\xB)\|$ for all feasible $\xB$ is bounded.
	\item The optimal objective value, denoted as $f_{\min}$, exists and $f_{\min}>-\infty$.
\end{enumerate}

By Corollary 3.1 of \citet{zhang2018convergence}, \method{} converges to an $\epsilon$-stationary point with the number of mirror descent iterations $\OM(\frac{1}{\epsilon^2})$.

\begin{flushright}
	$\blacksquare$
\end{flushright}

\paragraph{Proof of Proposition \ref{prop:K=1}}
When $K=1$, the \sis{} matrix can be rewritten as
\begin{equation*}
	\SB(\TB)=-t\WB^\src\TB\WB^\tar+t(\WB^\src\otimes\oneB+\oneB\otimes\WB^\tar-\WB^\src\TB\WB^\tar).
\end{equation*}
Note that $\tilde{\NM}_1^\src(i;\pi)\cap\NM_1^\tar(i')=\{j'|W_{ij}^\src T_{jj'}W_{i'j'}\neq 0\}$. For $\TB\in\Big\{\TB\in\{0,1\}^{V\times V}|\TB\oneB=\oneB,\TB^\top\oneB=\oneB\Big\}$, we have
\begin{equation*}
	|\tilde{\NM}_1^\src(i;\pi)\cap\NM_1^\tar(i')|=[\WB^\src\TB\WB^\tar]_{ii'}.
\end{equation*}
Since
\begin{equation*}
	|\tilde{\NM}_1^\src(i;\pi)\cup\NM_1^\tar(i')|=|\tilde{\NM}_1^\src(i;\pi)|+|\NM_1^\tar(i')|-|\tilde{\NM}_1^\src(i;\pi)\cap\NM_1^\tar(i')|,
\end{equation*}
we have
\begin{equation*}
	\begin{aligned}
		-\masis(i,i';\TB)&=t[\WB^\src\TB\WB^\tar]_{ii'}-t[\WB^\src\otimes\oneB+\oneB\otimes\WB^\tar-\WB^\src\TB\WB^\tar]_{ii'}\\
		&=t|\tilde{\NM}_1^\src(i;\pi)\cap\NM_1^\tar(i')|-t|\tilde{\NM}_1^\src(i;\pi)\cup\NM_1^\tar(i')|
	\end{aligned}
\end{equation*}
\begin{flushright}
	$\blacksquare$
\end{flushright}

To prove Proposition \ref{prop:relationship with MNC}, we need the following lemma.

\begin{lemma}\label{lem:inequality}
	For $1\le a\le b$, $\frac{a}{b}\ge\frac{e^a}{e^b}$.
\end{lemma}
\textbf{Proof:}

Consider function $f(x)=x-\log x$.
The derivative $f'(x)=1-\frac{1}{x}\ge 0$, for all $x\ge 1$.
Therefore, $f(x)$ increases monotonically for all $x\ge 1$.

Thus, $b-\log b\ge a - \log a$ for $1\le a\le b$, which can be rearranged to $\frac{a}{b}\ge\frac{e^a}{e^b}$.

\begin{flushright}
	$\blacksquare$
\end{flushright}

We now prove Proposition \ref{prop:relationship with MNC}.

\paragraph{Proof of Proposition \ref{prop:relationship with MNC}.}

%When $K=1$ and $|\VM^\src|=|\VM^\tar|$,
%\begin{equation*}
%	\SB(\TB)=\frac{\exp\big(t\WB^\src\TB\WB^\tar\big)}{\exp\big(t(\WB^\src\oneB\otimes\oneB+\oneB\otimes\WB^\tar\oneB-\WB^\src\TB\WB^\tar)\big)}.
%\end{equation*}
%By Theorem 4.1 of \citet{heimann2021refining}, for binary matching matrix $\TB\in\PM^f$,
%we have $|\tilde{\NM}_1^\src(i;\pi)\cap\NM_1^\tar(i')|=[\WB^\src\TB\WB^\tar]_{ii'}$ and $|\tilde{\NM}_1^\src(i;\pi)\cup\NM_1^\tar(i')|=[\WB^\src\oneB\otimes\oneB+\oneB\otimes\WB^\tar\oneB-\WB^\src\TB\WB^\tar]_{ii'}$.
%Therefore, $\maQuan(i,i';\TB)=\frac{\exp\Big(t|\tilde{\NM}_1^\src(i;\pi)\cap\NM_1^\tar(i')|\Big)}{\exp\Big(t|\tilde{\NM}_1^\src(i;\pi)\cup\NM_1^\tar(i')|\Big)}$.
%
%By Lemma \ref{lem:inequality}, when $|\tilde{\NM}_1^\src(i;\pi)\cup\NM_1^\tar(i')|\ge 1$, we have $\maQuan(i,i';\TB)\le\MNC(i,i';\pi)$.

By Proposition \ref{prop:K=1}, when $K=1$ and $\TB\in\Big\{\TB\in\{0,1\}^{V\times V}|\TB\oneB=\oneB,\TB^\top\oneB=\oneB\Big\}$,
\begin{equation*}
	\exp\big(-\masis(i,i';\TB)\big)=\frac{\exp\Big(t|\tilde{\NM}_1^\src(i;\pi)\cap\NM_1^\tar(i')|\Big)}{\exp\Big(t|\tilde{\NM}_1^\src(i;\pi)\cup\NM_1^\tar(i')|\Big)}.
\end{equation*}
By Lemma \ref{lem:inequality}, when $|\tilde{\NM}_1^\src(i;\pi)\cap\NM_1^\tar(i')|\ge 1$ and $t=1$, we have the result.

\begin{flushright}
	$\blacksquare$
\end{flushright}



==> local_topology arxiv/sections/related.tex <==
%要呼应intro里，没有side information，设计matching cost会很难。同时要讲一下SI的设计可以融合side information
\paragraph{Matching attributed graphs.}
Deep learning-based methods take as input the node/edge attributes of the graphs and learn node embeddings suitable for graph matching \citep{zanfir2018deep,fey2019deep,wang2019learning,sarlin2020superglue,wang2020combinatorial,yan2020learning}.
These supervised methods, however, require a large amount of anchor links that are often not available in practice.
Optimal transport-based methods exploit structural information and match graphs in an unsupervised manner \citep{maretic2019got,xu2019gromov,chowdhury2019gromov}.
To further incorporate node attributes,
Fused Gromov-Wasserstein distance-based methods are proposed to exploit both node attributes and structure information \citep{titouan2019optimal,barbe2020graph}.
Node or edge attributes can be incorporated into the design of \sis{}.

\paragraph{Graph distance.}
%\Realworld{} data are often structured and represented as graphs.
Comparison among graphs is ubiquitous in analyzing graph-structured data.
Spectral distances usually do not take into account all the structural information,
focusing only on the
Laplacian matrix eigenvectors and ignoring a large portion of the structure encoded in eigenvectors \citep{jovanovic2012spectral,gera2018identifying}.
The cut distance \citep{lovasz2012large} and the graph edit distance \citep{bougleux2017graph,raveaux2021unification} require solving difficult discrete optimization problems.
%By modelling graphs as probability distributions,
%transportation distances between graphs \citep{maretic2019got,titouan2019optimal,barbe2020graph} can be effectively and efficiently calculated by borrowing tools from optimal transport theory \citep{villani2008optimal}.
Another family of graph distances that is closely related to this paper is the graph diffusion distance \citep{hammond2013graph,tsitsulin2018netlsd,scott2021graph}.
\citeauthor{hammond2013graph} \citeyear{hammond2013graph} assume the nodes of the two graphs are already matched and calculate the graph diffusion distance.
\citeauthor{scott2021graph} \citeyear{scott2021graph} extend \citet{hammond2013graph}'s work and address the graph matching problem.
Their method involves solving a three-level optimization problem and estimates the node correspondence in the innermost problem by matching eigenvalues of the heat diffusion kernel matrix.
Note that our Eq. (\ref{eq:real objective}) also defines a distance between two graphs.

==> local_topology arxiv/sections/si.tex <==
Based on the local neighborhoods of node $i$ and node $i'$,
they can be embedded into a $V$-dimensional space,
which yields embedding vectors $\zB_{i}$ and $\zB_{i'}$ respectively.
The $j$-th dimension of $\zB_{i}$ (resp. $j'$-th dimension of $\zB_{i'}$) models the distance between $i$ and $j$ (resp. $i'$ and $j'$).
%Note that the coordinate axes of $\zB_{i}$ and $\zB_{i'}$ are not in correspondence.
In this paper,
we instantiate the embeddings based on HDW, i.e., $\zB_{i}=\BB[i:]$ and $\zB_{i'}=\BB[i':]$

Given transport plan $\TB\in\Pi(\oneB,\oneB)$,
we model the \si{} (\sis{}) of a pair of nodes $(i, i')\in\VM^\src\times\VM^\tar$ as a \emph{transport distance}
\begin{equation}
	\masis(i,i';\TB)=\sum_{j=1}^{V}\sum_{j'=1}^{V}T_{jj'}(B_{ij}^\src-B_{i'j'}^\tar)^2.
\end{equation}
\begin{wrapfigure}{r}{0.5\textwidth}%图放后面
	\begin{subfigure}[b]{0.295\textwidth}
		\includegraphics[width=\textwidth]{imgs/topology_violation.pdf}
		\caption{The \si{} of node pair $(A,a)$.}\label{fig:violation part}
	\end{subfigure}
	~
	\begin{subfigure}[b]{0.185\textwidth}
		\includegraphics[width=\textwidth]{imgs/topology_conservation.pdf}
		\caption{Maximal structural consistency.}\label{fig:conservation part}
	\end{subfigure}
	\caption{The inconsistency of one-hop neighborhood for node pair $(A,a)$. The gray ovals indicate the one-hop neighbors of $A$ and $a$ respectively. The dashed lines denote the matching of $A$ and its one-hop neighbors, and mismatches exist  in Figure \ref{fig:violation part} and thus structural inconsistency occurs.}\label{fig:topology violation}
\end{wrapfigure}
We illustrate $\masis(A,a)$ when $K=1$ in Figure \ref{fig:topology violation}.
Here the transport plans are depicted by the thin dashed lines and we omit them in \sis{}.
In Figure \ref{fig:violation part}, node $B$ (resp. $C$) is wrongly matched to node $c$ (resp. $b$).
Nodes $A$ and $B$ ($a$ and $b$) are connected by an edge while no edge connects $a$ and $c$($A$ and $C$),
which is depicted by the two red(yellow) circles.
Therefore, structural inconsistency incurs.
In Figure \ref{fig:conservation part}, node $A$ and its one-hop neighbors are correctly matched,
which leads to $\masis(A,a)=0$. 

One can derive a \sis{} matrix.
The \sis{} for all node pairs $(i, i')$ given the matching matrix $\TB$, can be written as a matrix $\SB=[S_{ii'}]$ such that $\masis(i,i';\TB)=S_{ii'}$ as
\begin{equation*}
	\SB(\TB)=-2\BB^\src\TB\BB^\tar+h(\BB^\src)\oneB\otimes\oneB+\oneB\otimes h(\BB^\tar)\oneB,
\end{equation*}
where $h$ denotes the element-wise square and $\otimes$ is the outer product of two vectors.
We further define the structural inconsistency of true counterparts (CSI) as
\begin{equation}\label{eq:csi}
	\macsi(i;\TB)=\masis(i,\pi^*(i);\TB),
\end{equation}
where $\pi^*$ is the true matching.

\sis{} is closely related to alignment accuracy.
On the one hand, if node pair $(i,\hat{i})$ have zero \sis{} values, $\hat{i}$ either is the true counterpart $\pi^*(i)$ or have the same local topology as $\pi^*(i)$,
which is formalized in the following theorem.
\begin{theorem}\label{thm:indistinguishable}
	Assume $\GM^\src$ and $\GM^\tar$ are isomorphic and there exists $\TB$ that yields $\masis(i,\hat{i};\TB)=0$.
	Then, if $\hat{i}\neq\pi^*(i)$, $\NM_k^\tar(\hat{i})$ and $\NM_k^\tar\big(\pi^*(i)\big)$ are isomorphic for all $k\le K$.
\end{theorem}
An example of Theorem \ref{thm:indistinguishable} is matching two star graphs, each consisting of one center node connected to $n-1$ peripheral nodes \citep{heimann2021refining}.
Matching peripheral nodes to each other in any order leads to zero \sis{}'s,
whatever the true correspondence of the peripheral nodes is.
This inspires us to use larger neighborhoods to improve the performance, since $\NM_{k+1}^\tar(\hat{i})$ and $\NM_{k+1}^\tar\big(\pi^*(i)\big)$ may not be isomorphic when $\NM_k^\tar(\hat{i})$ and $\NM_k^\tar\big(\pi^*(i)\big)$ are.

On the other hand, if $\GM^\src$ is isomorphic to $\GM^\tar$ up to a few noisy or missing edges (the vetex sets remain the same),
$\macsi\big(i;\TB^*\big)$ values are low where $\TB^*=[T_{ii'}^*]$ is matrix form of true matching.
This is stated in the following theorem.
\begin{theorem}\label{thm:principle}
	Let $\DeltaB_k\in\RBB^{V\times V}$ denote the perturbation to the edge structure, which is given by $\DeltaB_{k}=(\LB^\src)^k-(\tilde{\LB}^\tar)^k$ where $\tilde{\LB}^\tar=\TB^*\LB^\tar\TB^{*\top}$ is the Laplacian matrix of the registered target graph.
	Assume that for all $i$,
	the perturbation to the local neighborhood is bounded as $\epsilon_k=\max_i\sum_{j\in\NM_k^\src(i),j'\in\NM_k^\tar(\pi^*(i))}|\Delta_{k,jj'}|^2$
	Then $\macsi\big(i;\TB^*\big)$ can be bounded from above as follows:
	\begin{equation*}
		\macsi\big(i;\TB^*\big)\le K\sum_{k=1}^{K}\Big(\frac{(-t)^k}{k!}\Big)^2\epsilon_k,
	\end{equation*}
	where $t$ is the propagation time.
\end{theorem}
%$\macsi\big(i;\TB^*\big)$ is a small quantity.
%To capture local topology, the propagation time $t$ is a small value \citep{tsitsulin2018netlsd,donnat2018learning}.
%For a fixed $K$, when the perturbation to the structure is small,
%$\macsi\big(i;\TB^*\big)$ is bounded and close to $0$,
%which justifies the our method design.

Note that the propagation time $t$ is often set to a small value in order to capture the local topology  \citep{tsitsulin2018netlsd,donnat2018learning}. 
Thus, for a fixed $K$, when the perturbation $\epsilon_k$ is  small,  $\macsi (i; \TB^* )$ has a small upper bound and even is close enough to 0.
It is reasonable to conjecture that keeping decreasing CSI will lead to an optimal result, which is embodied in our method design.

%The small-world property of real graphs suggests that a moderate $K$ is enough in practice \citep{watts1998collective}.

%For $i'\neq\pi^*(i)$, $\masis\big(i,i';\TB^*\big)=\sum_{j=1}^{V}(B_{ij}^\src-B_{i'\pi^*(j)}^\tar)^2$ is usually large unless $i'$ is structurally similar to $\pi^*(i)$.

% for a fixed K, justify. K too large

==> local_topology arxiv/sections/theory.tex <==
In this section, we first prove that iteration (\ref{eq:iteration}) can reduce $\macsi(i;\TB)$ for all $i$ under suitable assumptions.
Then the convergence of \method{} is proved.
We also discuss its relationship to state-of-the-art methods.

With appropriate $\eta^{(\tau)}$, iteration \ref{eq:iteration} can reduce alignment score $T_{ii'}$ if $\masis(i,i';\TB^{(\tau)})$ is high,
which is formalized in the following lemma.
\begin{lemma}\label{lem:mirror descent assumptions}
	If $\frac{1}{T_{ii^*}^{(\tau)}}\exp\Big(\eta^{(\tau)}\macsi(i;\TB^{(\tau)})\Big)\le\exp\Big(\eta^{(\tau)}\masis(i;i';\TB^{(\tau)})\Big)$ where $i^*=\pi^*(i)$ and $i'\neq i^*$, $T_{ii'}^{(\tau+1)} < T_{ii'}^{(\tau)}$.
\end{lemma}


We now state our main theorem.
\begin{theorem}\label{thm:each step}
	If $T_{ii'}^{(\tau+1)} < T_{ii'}^{(\tau)}$ for all $i$ and $i'\neq i^*$,
	then $\macsi(i;\TB^{(\tau+1)})< \macsi(i;\TB^{(\tau)})$.
\end{theorem}
Combining Lemma \ref{lem:mirror descent assumptions} and Theorem \ref{thm:each step}, if we have $\frac{1}{T_{ii^*}^{(\tau)}}\exp\Big(\eta^{(\tau)}\macsi(i;\TB^{(\tau)})\Big)\le\exp\Big(\eta^{(\tau)}\masis(i;i';\TB^{(\tau)})\Big)$ for all $i$ and $i'\neq \hat{i}$, we can reduce $\macsi(i;\TB)$ at iteration $\tau$.

By establishing the relationship between \method{} and optimal transport based methods, we can borrow the convergence result of mirror descent and prove that \method{} converges as follows.
\begin{theorem}\label{thm:md}
	\method{} converges to an $\epsilon$-stationary point with the number of mirror descent iterations $\OM(\frac{1}{\epsilon^2})$.
\end{theorem}
The main steps of the proof follow \citet{zhang2018convergence}.
We further remark that the true matching matrix $\TB^*$ is a fixed point of update (\ref{eq:iteration}).
%\begin{theorem}\label{thm:fixed point}
%	$\TB^*$ is a fixed point for iteration (\ref{eq:iteration}).
%\end{theorem}

%\begin{theorem}\label{thm:each step}
%	When the following assumptions hold:
%	\begin{enumerate}
%		\item For all $i\in\VM^\src$, there exists $\hat{i}\in\VM^\tar$, such that $\NM_k^\src(i)$ is isomorphic to $\NM_k^\tar(\hat{i})$,
%		\item\label{assu:all decrease} $T_{ii'}^{(\tau+1)} < T_{ii'}^{(\tau)}$ for all $i$ and $i'\neq \hat{i}$,
%	\end{enumerate}
%	then $\masis(i,\hat{i};\TB^{(\tau+1)})< \masis(i,\hat{i};\TB^{(\tau)})$.
%\end{theorem}

\paragraph{Computational complexity.}
The complexity for calculaing the heat diffusion wavlets is $\OM(KV^3)$.
Due to the two matrix multiplication steps of the term $\BB^\src\TB\BB^\tar$,
calculating the gradient involves computational complexity $\OM(V^3)$.
Note that the matrix multiplication is highly parallelizable and well-suited to modern computing architectures like GPUs.
$\OM(V^2)$ cost is induced by the matrix-vector multiplication in the projection operation.
Therefore, if we run projected mirror descent for $N$ iterations, each of which involves $T$ matrix-vector multiplications in the projection,
$\OM\big(NTV^2+(N+K)V^3\big)$ computational cost is required in learning the matching matrix.
Such complexity is of the same order as state-of-the-art methods like \citet{xu2019gromov,konar2020graph,scott2021graph,heimann2021refining},
and lower than \citet{neyshabur2013netal,malod2015graal,fan2020spectral}.
Considering the sparsity of edges in \realworld{} graphs,
the complexity can be reduced to $\OM\big(NTV^2+(N+K)VE\big)$ where $E=\max\{|\EM^\src|,|\EM^\tar|\}$.



\subsection{Connection to GWL \citet{xu2019gromov}}
%OT-based methods exploit the geometric properties of the metric spaces that underlie the graphs.
%The source graph $\GM^\src$ and the target graph $\GM^\tar$ are modelled as two probability distributions $\muB^\src=[\mu^\src_i]$ and $\muB^\tar=[\mu^\tar_i]$ respectively,
%where
%\begin{equation*}
%	\mu^z_i=\frac{\sum_{j=1}^{|\VM^z|} W_{ij}^z}{\sum_{i=1}^{|\VM^z|}\sum_{j=1}^{|\VM^z|}W_{ij}^z}, \text{ for }z=\src,\tar.
%\end{equation*}
%Basically, the node correspondence is estimated by calculating the transport plan of the Gromov-Wasserstein distance that is defined as $GW(\muB^\src,\muB^\tar)=\min_{\TB\in\Pi(\muB^\src,\muB^\tar)}\ell(\TB)$, where
%\begin{equation}\label{eq:Xu GW}
%	\ell(\TB)=\sum_{i=1}^{|\VM^\src|}\sum_{j=1}^{|\VM^\src|}\sum_{i'=1}^{|\VM^\tar|}\sum_{j'=1}^{|\VM^\tar|}(B_{ij}^\src-B_{i'j'}^\tar)^2T_{ii'}T_{jj'},
%\end{equation}
%and $\Pi(\pB,\qB)=\{\TB\in\RBB_+^{m\times n}|\TB\oneB_n=\pB,\TB^\top\oneB_m=\qB\}$.
%Node $i\in\VM^\src$ is matched to $\hat{i}\in\VM^\tar$,
%where $\hat{i}=\argmax_{i'}[T^*_{ii'}]$ and $\TB^*=[T^*_{ii'}]$ attains the minimum of Eq. (\ref{eq:Xu GW}).

The gradient that arises from Problem (\ref{eq:Xu GW}) \citep{xu2019gromov,xu2019scalable,titouan2019optimal,barbe2020graph} and has the following form:
\begin{equation}\label{eq:gradient Xu}
	\nabla\ell(\TB)=h(\BB^\src)\oneB\otimes\muB^\src+\oneB\otimes h(\BB^\tar)\muB^\tar-2\BB^\src\TB\BB^\tar,
\end{equation}
where $h$ denotes the element-wise square and $\otimes$ is the outer product of two vectors \citep{peyre2016gromov}.
Note that if we set $\mu_i^z=1$ for all $i$ and $z=\src,\tar$, (\ref{eq:gradient Xu}) is identical to (\ref{eq:gradient Ours}).

GWL uses \emph{proximal point method} to solve Problem (\ref{eq:Xu GW}) \citep{xu2019gromov}.
If one single mirror descent step is adopted to solve the sub-problem and the marginals are set as $\mu_i^z=1$,
the proximal point method is identical to our mirror descent method.



\subsection{Connection to RefiNA \citet{heimann2021refining}}
When $K=1$, the pairwise \sis{} has a more intuitive interpretation.
\begin{proposition}\label{prop:K=1}
	When one only uses one-hop neighborhood information (i.e., $K=1$),
	\begin{equation*}
		\begin{aligned}
			\exp\big(-\masis(i,i';\TB)\big)=\frac{\exp\Big(t|\tilde{\NM}_1^\src(i;\pi)\cap\NM_1^\tar(i')|\Big)}{\exp\Big(t|\tilde{\NM}_1^\src(i;\pi)\cup\NM_1^\tar(i')|\Big)},
		\end{aligned}
	\end{equation*}
	where $\TB\in\Big\{\TB\in\{0,1\}^{V\times V}|\TB\oneB=\oneB,\TB^\top\oneB=\oneB\Big\}$, $\tilde{\NM}_k^\src(i;\pi)$ is the set of nodes onto which $\pi$ maps $i$'s neighbors $\tilde{\NM}_k^\src(i;\pi)=\{j'\in\VM^\tar|\exists j\in\NM_k^\src(i) \st \pi(j)=j'\}$, and the bijective is given by $\pi(i)=\argmax_{i'}[T_{ii'}]$.
\end{proposition}

\citeauthor{chen2020cone} \citeyear{chen2020cone} and \citeauthor{heimann2021refining} \citeyear{heimann2021refining} define a similar quantity.
Specifically, the \emph{matched neighborhood consistency} (MNC) of node $i$ in $\GM^\src$ and node $i'$ in $\GM^\tar$ is the Jaccard similarity of the sets $\tilde{\NM}_1^{\src}(i;\pi)$ and $\NM_{1}^\tar(i')$, i.e., $\operatorname{MNC}(i, i';\pi)=\frac{\left|\tilde{\NM}_1^{\src}(i;\pi) \cap \NM_{1}^\tar(i')\right|}{\left|\tilde{\NM}_1^{\src}(i;\pi) \cup \NM_{1}^\tar(i')\right|}$.
$\masis(i,i';\TB)$ and $\operatorname{MNC}(i, i';\pi)$ can be related as follows.
\begin{proposition}\label{prop:relationship with MNC}
	When propagation time $t=1$ and $\tilde{\NM}_1^{\src}(i;\pi) \cap \NM_{1}^\tar(i')$ is not empty,
	\begin{equation*}
		\exp\big(-\masis(i,i';\TB)\big) \le \MNC(i,i';\pi).
	\end{equation*}
\end{proposition}

According to Proposition \ref{prop:relationship with MNC}, Lemma \ref{lem:mirror descent assumptions} and Theorem \ref{thm:each step}, \method{} with $K=1$ and $t=1$ can also be viewed as increasing a soft version of MNC values, which is positively related to MNC and should also be high/low for accurate/inaccurate matching.
Combined with the description in Sec. \ref{sec:method}, \method{} can be regarded as the first OT-based method that are guaranteed to increase MNC in each iteration in the graph matching literature.
In addition, by characterizing the structure of a larger neighborhood via HDW, we alleviate the problem of near structural indistinguishability and improves the matching performance.

%Besides, we also show that our method increases a soft version of MNC values, which is positively related to MNC and should also be high/low for accurate/inaccurate matching.
%\method{} can be regarded as the first OT-based method that are guaranteed to increase MNC in each iteration in the graph matching literature.

==> local_topology arxiv/sections/topology.tex <==
%We present our topological view for OT-based graph matching methods by three steps:
%1) Each entry of the gradient with respect to the transport plan can be viewed as the topology violation of the corresponding node pair and existing OT-based graph matching methods increase the alignment scores of node pairs with low violation values.
%2) Under suitable assumptions,
%such procedure can reduce the topology violation of matched node pairs.
%%and increase the probability that true node pairs are matched.
%3) Low topology violation of all matched node pairs is a necessary condition for accurate matching.

We present our topological view for OT-based graph matching methods by three steps:
1) Each entry of the gradient with respect to the transport plan, denoted as $G_{ii'}(\TB)$, can be viewed as the topology violation of node pair $(i,i')$;
2) Because of the feasible domain, gradient-based methods increase $T_{ii'}$ if $G_{ii'}(\TB)$ is large and decrease $T_{ii'}$ if $G_{ii'}(\TB)$ is small,
so that overall topology violation is reduced;
3) Under suitable assumptions,
the topology violation values of matched node pairs, denoted as $G_{i\hat{i}}$'s where node $i$ is matched to node $\hat{i}$, tend to $0$,
which is a sufficient and necessary condition for matching structurally distinguishable nodes.

\subsection{Topology Violation and OT}

OT-based methods adjust the transport plan dynamically according to the topology violation.
%Following the definition of \emph{measure networks} \citep{chowdhury2019gromov,xu2019gromov},
Mainstream methods assign two distributions $\muB^\src=[\mu^\src_i]$ and $\muB^\tar=[\mu^\tar_i]$ to the source graph $\GM^\src=(\VM^\src,\EM^\src,\WB^\src)$ and the target graph $\GM^\tar=(\VM^\tar,\EM^\tar,\WB^\tar)$ respectively \citep{xu2019gromov,xu2019scalable,chowdhury2019gromov,titouan2019optimal,barbe2020graph},
where
\begin{equation*}
	\mu^z_i=\frac{\sum_{j=1}^{|\VM^z|} W_{ij}^z}{\sum_{i=1}^{|\VM^z|}\sum_{j=1}^{|\VM^z|}W_{ij}^z}, \text{ for }z=\src,\tar.
\end{equation*}
%Without loss of generality, we assume $|\VM^\src|\le|\VM^\tar|$.
A cost matrix $\CB^z=[C_{ij}^z]\in\RBB^{|\VM^z|\times|\VM^z|}$ is further defined with each $C_{ij}^z$ characterizing the dissimilarity between vertices $i$ and $j$.
%for example,
%$C_{ij}^z=\frac{1}{1+W_{ij}^z}$ \citep{xu2019gromov}.%例子都写出来，别管全局和局部
The GW distance between $\GM^\src$ and $\GM^\tar$ is then defined as
\begin{equation}\label{eq:Xu GW}
		GW(\muB^\src,\muB^\tar)=\min_{\TB\in\Pi(\muB^\src,\muB^\tar)}\sum_{i=1}^{|\VM^\src|}\sum_{j=1}^{|\VM^\src|}\sum_{i'=1}^{|\VM^\tar|}\sum_{j'=1}^{|\VM^\tar|}(C_{ij}^\src-C_{i'j'}^\tar)^2T_{ii'}T_{jj'}.
\end{equation}
%The transport plan $\TB^*$ that attains the minimum indicates the node correpsondence across the two graphs.
Node $i\in\VM^\src$ is matched to $\hat{i}\in\VM^\tar$ where $\hat{i}=\argmax_{i'}T^*_{ii'}$ and $\TB^*=[T^*_{ii'}]$ attains the minimum of Eq. (\ref{eq:Xu GW}).

Existing methods update the transport plan using the gradient that arises from Problem (\ref{eq:Xu GW}) \citep{xu2019gromov,xu2019scalable,titouan2019optimal,barbe2020graph} and the gradient has the following form:
\begin{equation}
	\GB(\TB)=h(\CB^\src)\oneB\otimes\oneB+\oneB\otimes h(\CB^\tar)\oneB-2\CB^\src\TB\CB^\tar,
\end{equation}
where $h$ denotes the element-wise square and $\otimes$ is the outer product of two vectors \citep{peyre2016gromov}.

The gradient with respect to the transport plan $\GB(\TB)=[G_{ii'}(\TB)]$ admits topological interpretation.
In particular, each entry can be written as the transport distance,
%between two discrete measures induced by nodes $i$ and $i'$ respectively,
\begin{equation*}\label{eq:gradient interpretation}
	G_{ii'}(\TB)=\sum_{j=1}^{|\VM^\tar|}\sum_{j'=1}^{|\VM^\tar|}T_{jj'}(C_{ij}^\src-C_{i'j'}^\tar)^2,%局部还是全局？和C取值有关系
\end{equation*}
and can be interpreted as the \emph{violation} of the local topology of node $i\in\VM^\src$ and $i'\in\VM^\tar$ given the current transport plan $\TB$.
%Exising methods gradually improve the matching accuracy by 
Since the transport plan satisfies the constraints $\TB\in\Pi(\muB^\src,\muB^\tar)$,
existing methods increase $T_{jj'}$ with small $G_{ii'}(\TB)$ in each iteration to reach a matching consensus in local neighborhoods between graphs.
This is essentially in the same spirit as \citeauthor{fey2019deep} \citeyear{fey2019deep}'s work,
which matches attributed graphs in a supervised manner.

\subsection{Reducing Topology Violation}

%Increasing the alignment score $T_{ii^*}$ where node $i^*$ is the true counterpart of node $i$, can in turn reduce the transport distance $G_{ii^*}(\TB)$, i.e., improve the topology conservation of $(i,i^*)$.
%This also increases the possibility that $i^*$ is matched to $i$. 
%Denote 
%Increasing the alignment score of true node pairs can in turn reduce the transport distance $G_{ii^*}(\TB)$.
%\begin{proposition}\label{prop:each step}
%	Denote the recurrence by $\TB^{(\tau+1)}=\iota\big(\TB^{(\tau)}\big)$.
%	For isomorphic graphs,
%	the transport distances of true node pairs decrease at iteration $\tau$, $G_{ii^*}(\TB^{(\tau+1)})\le G_{ii^*}(\TB^{(\tau)})$,
%	if $T_{ii'}^{(\tau+1)}\le T_{ii'}^{(\tau)}$ for all $i$ and $i'\neq i^*$.
%\end{proposition}


Increasing the alignment score $T_{ii'}$ if the topology violation $G_{ii'}(\TB)$ is small,
can in turn reduce the topology violation of matched node pairs,
when matched node pairs have similar local topology.
We first formalize the concept of local neighborhoods.
\begin{definition}[$k$-hop neighborhood]
	The $k$-hop neighborhood of node $i$ in graph $z$, denoted by $\NM_k^z(i)$, is the subgraph of $\GM^z$ induced by all nodes that are $k$ or fewer hops away from node $i$, where $z=\src,\tar$.
\end{definition}


\begin{proposition}\label{prop:each step}
	Denote the recurrence by $\TB^{(\tau+1)}=\iota\big(\TB^{(\tau)}\big)$.
	When the following assumptions hold:
	\begin{enumerate}
		\item $\GM^\src$ and $\GM^\tar$ are isomorphic,
		\item for all $i\in\VM^\src$, $\NM_k^\src(i)$ is isomorphic to $\NM_k^\tar(\hat{i})$ where $\hat{i}$ is the matched node for $i$, $\hat{i}=\argmax_{i'}T_{ii'}$,
		\item the cost matrix quantifies the local topology, i.e., if node j is more than $k$ hops away from node $i$, $C_{ij}^z=\bar{\Psi}$ is large for $z=\src,\tar$,
		\item $T_{ii'}^{(\tau+1)}\le T_{ii'}^{(\tau)}$ for all $i$ and $i'\neq \hat{i}$,
	\end{enumerate}
	the transport distances of all matched node pairs decrease at iteration $\tau$, $G_{i\hat{i}}(\TB^{(\tau+1)})\le G_{i\hat{i}}(\TB^{(\tau)})$.%会不会降到大于0的一个数就停下来了
\end{proposition}

In Sec. \ref{sec:method},
we propose a mirror descent-based method that match graphs by reducing topology violation.

%\subsection{Necessity of Small Topology Violation}
Low transport distance for all matched node pairs is a necessary condition for accurate alignment.

On the one hand, accurate matching entails low transport distance for matched node pairs.
For all true node pairs $(i,i^*)$ and the optimal transport plan $\TB^*=\argmin_{\TB\in\Pi(\muB^\src,\muB^\tar)}\sum_{ii'jj'}(C_{ij}^\src-C_{i'j'}^\tar)^2T_{ii'}T_{jj'}$, the transport distance is small, which is stated in the following proposition.
\begin{proposition}\label{prop:transport distance}
	For isomorphic graphs and $C_{ij}^z=\frac{1}{1+W_{ij}^z}$,%C不止可以取这种形式
%	denote the true matching matrix by $\TB^*$,
	the transport distance of all matched node pairs $(i,i^*)$ where $i^*=\argmax_{i'}T^*_{ii'}$ is 0,
	\begin{equation*}
		G_{ii^*}(\TB^*)=0,
	\end{equation*}
	while for node $i'\neq i^*$, the transport distance is generally large
	\begin{equation*}
		G_{ii'}(\TB^*)=\sum_{j=1}^{|\VM^\src|}\mu_j^\src(C_{ij}^\src-C_{i'j^*}^\tar)^2,
	\end{equation*}
	where $j^*=\argmax_{j'}T^*_{jj'}$.
\end{proposition}
Therefore, we aim to estimate the node correspondence by minimizing the transport distance for matched node pairs in this paper.

On the other hand, misalignment may still occur even if the transport distances for all matched node pairs are low.
This is due to (near) structural indistinguishability.
To illustrate this, consider an extreme case of matching two star graphs, each consisting of one center node connected to $n-1$ peripheral nodes \citep{heimann2021refining}.
Matching peripheral nodes to each other in any order leads to zero transport distances,
whatever the true correspondence of the peripheral nodes is.
Distinguishing such nodes from pure graph topology is impossible.
%In many cases, however, one may alleviate (near) structural indistinguishability by taking a larger neighborhood into account.


==> sections/checklist.tex <==
%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%  \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} See Sec. \ref{sec:experimental setup}.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{} See Figure \ref{fig:full main}.
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} See Sec. \ref{sec:experimental setup}.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{} See Sec. \ref{sec:experimental setup} and the readme file in the code submission.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/introduction-v1.tex <==
Graph matching (network alignment) aims to identify the correspondence of nodes across two related graphs,
by minimizing the sum of pair-wise matching costs of corresponding nodes/edges.
It has many applications,
such as
linking user accounts in social platforms \citep{shu2017user,wang2019user},
aligning entities in knowledge graphs \citep{sun2020knowledge,pei2020rea},
and matching keypoints across two images \citep{sarlin2020superglue,wang2020zero},
to name a few.

%The choice of matching costs is critical to the performance of graph matching.%when side available，设计matching costs更加困难如果只有拓扑连接，
%Originally, matching costs are mainly calculated using handcrafted features that rely%不要mainly
%heavily on expert knowledge \citep{patro2012global,sun2015simultaneous,mamano2017sana}.
%Recently, end-to-end deep learning methods for graph matching are proposed
%to automatically learn the node embedding-based matching
%costs \citep{zanfir2018deep,fey2019deep,wang2019learning,sarlin2020superglue,wang2020combinatorial}.
%These methods, however, require side information including node or edge features, and a large amount of anchor links (labelled node correspondences).
%In practice, side information are often not available \citep{snapnets,heimann2021refining}.%however in many tasks，没有side information使得更加复杂更难，只能通过
%Under such circumstance,
%the node correspondence is often estimated on the sole basis of the network topologies of the two graphs.%连接关系，后面这句是主句。

The choice of matching costs is critical to the performance of graph matching.
%and designing matching costs is more challenging when node or edge features are not available.
When  node/edge side information, e.g. attributes, are available,
one can rely on expert knowledge to design handcrafted node embeddings for the calculation of matching costs
% matching costs are commonly calculated by using handcrafted features that rely heavily on expert knowledge 
\citep{zhang2016final,meng2016igloo}.
Recently, to alleviate the requirement of expert knowledge, 
end-to-end deep learning methods are proposed
to learn the node embedding automatically based on the \emph{anchor links} (labelled node correspondences)\citep{zanfir2018deep,fey2019deep,wang2019learning,sarlin2020superglue,wang2020combinatorial}.
However, in many tasks, side information and/or anchor links are not available \citep{snapnets,heimann2021refining}.
Under such circumstance,
These methodshowever, require side information including node or edge features, and a large amount of \emph{anchor links} (labelled node correspondences).
In many tasks, however, graphs are often unattributed \citep{snapnets,heimann2021refining}.
Under such circumstance,
the matching costs are often estimated on the sole basis of the network topologies of the two graphs.

%\citeauthor{heimann2021refining} \citeyear{heimann2021refining} theoretically demonstrates a close relationship between \emph{matched neighborhood consistency} (MNC) and the matching quality.
The seminal work of \citet{heimann2021refining} reveals the close connection between \emph{matched neighborhood consistency} (MNC) and the alignment accuracy.
In particular,
accurate alignment entails high MNC.
However, several limitations still remain:%紧密的关系，connection between
1) Their method, RefiNA, only considers the numerators of MNC values, which leads to a gap between their method and their theoretical analysis;
2) RefiNA only uses one-hop neighborhoods, which easily leads to (near) structural indistinguishability and misaligns nodes that have low degrees.

Recently, one line of works align graphs by borrowing tools from
optimal transport (OT),
which can match graphs in an unsupervised fashion \citep{memoli2011gromov,maretic2019got,xu2019gromov,titouan2019optimal,chowdhury2019gromov,barbe2020graph}.
These methods exploit the geometric properties of the metric spaces that underlie the graphs and exhibits good empirical performance.
Basically, the node correspondence is estimated by calculating the \emph{transport plan} of the Gromov-Wasserstein distance that captures the \emph{global} structural information \citep{barbe2020graph}.
However, it remains unknown how these OT-based methods exploit the \emph{local} topology to iteratively improve the matching accuracy and whether they conform to the MNC principle.
Besides, their alignment costs hinge on the one-hop neighborhood of each node, which leaves room for improvement.

%Recently, there has been significant interest in designing \emph{heat diffusion}-based methods to capture the structural information of graphs (eg. \citep{tsitsulin2018netlsd,berberidis2018adaptive,donnat2018learning,klicpera2019diffusion}). 
%The heat diffusion on a graph is the solution to the discrete heat equation \citep{kondor2002diffusion}.
%Intuitively, each node propagates a unit of energy over the graph and the local topology is characterized by the amount of energy that each neighboring node receives after a given time.
%It can be proved that nodes that share similar local topology have similar diffusion patterns \citep{donnat2018learning}.
%which also implies that heat diffusion is robust to small perturbations of the edge structure \citep{donnat2018learning,berberidis2018adaptive,klicpera2019diffusion}.
%The computational complexity of heat diffusion is linear in the number of edges \citep{defferrard2016convolutional,donnat2018learning}, thus allowing it to scale to \realworld{} graphs.
%Therefore, heat diffusion allows us to characterize the multi-hop neighborhood of each node and match node pairs that have similar local topological structures.
%Heat diffusion, however, is mainly used to fuse node attributes in attributed graphs instead of matching unattributed graphs in the graph matching literature \citep{li2019graph,barbe2020graph}.


%In this paper, we propose a novel graph matching method \method{} to tackle the challenging problem of matching two unattributed graphs without anchor links.
%Our method uses \emph{heat diffusion wavelet} (HDW) \citep{donnat2018learning} to characterize the structure of multi-hop neighborhoods (hence the name).
%Based on the captured structural information,
%we define a novel quantity, pairwise \si{} (\sis{}).%先提这个概念，比measure更弱的量criterion，揭示了和accuracy的关系。提出了新方法。可以很容易嵌入小波
%Our method improves the alignment scores of node pairs that have low \sis{} values in each iteration.

This paper considers the challenging problem of matching two unattributed graphs without anchor links.
A novel concept, \si{} (\sis{}), is defined to measure the correspondence quality of a node pair.
We reveal the connection between \sis{} values of predicted node counterparts and the matching quality.
Our method, \method{}, improves the alignment scores of node pairs that have low \sis{} values in each iteration.
By incorporating \emph{heat diffusion wavelet} \citep{donnat2018learning},
\method{} considers the multi-hop structural information and increases the distinguishability of nodes.

%Our contributions are summarized as follows.
%\begin{itemize}
%	\item \textbf{A new method.}%更符合，并且引入k.
%	A novel quantity, pairwise \si{} (\sis{}), is defined to evaluate the quality of the estimated node correspondence,
%	based on which we propose a new graph matching method named \method{}.
%	By taking a larger neighborhood into account,
%	the (near) structural indistinguishability problem is alleviated.
%	\item \textbf{Theoretical analysis.}% corresponding SI 和MNC的关系，理论分析要有形容词，对应关系
%	We theoretically analyze the relationship between \sis{} and the alignment accuracy.
%	We prove that \method{} can reduce \sis{} under suitable assumptions.
%	The convergence of \method{} to a first-order stationary point is proved and the true matching matrix is proved to be one fixed point of the update.
%	We demonstrate that our method is essentially the mirror descent method for solving the Gromov-Wassetstein distance and thus provides a local topological perspective for OT-based methods.
%	We also reveal that our method increases a lower bound of MNC values.
%\end{itemize}

Our contributions are summarized as follows.
\begin{itemize}
	\item We propose a new graph matching method named \method{} to match two unattributed graphs without anchor links.
	Compared to RefiNA \citep{heimann2021refining},
	\method{} is more conforming to the MNC principle.
	By taking a larger neighborhood into account,
	\method{} increases the distinguishability of nodes and improves the matching quality.
	\item We conduct theoretical analysis for \method{}.
	We reveal that \sis{} have a close relationship to matching accuracy.
	On the one hand, if a pair of nodes incurs zero \sis{}, they have the same local topology.
	On the other hand, \sis{} values of true counterparts are bounded and close to zero.
	Under suitable assumptions, \method{} can reduce \sis{} values of true counterparts.
	We demonstrate that \method{} is essentially a mirror descent method for solving the Gromov-Wassetstein distance and provides a local topological perspective for OT-based methods.
	We also prove that our method increases a lower bound of MNC values, instead of increasing the numerators.
\end{itemize}

Extensive experimental results demonstrate that the proposed method outperforms state-of-the-art methods.
The rest of the paper is organized as follows.
In Sec. \ref{sec:preliminary}, we review the background and discuss the relationship between \sis{} and matching accuracy.
Based on \sis{}, a new graph matching method \method{} is proposed in Sec. \ref{sec:method}.
We give theoretical analysis in Sec. \ref{sec:theory}.
Due to the limited space, all proof are given in the appendix.
Experimental results are demonstrated in Sec. \ref{sec:experiment} and the appendix.



%Graph matching is a key step for many graph analysis tasks including
%%	graph isomorphism test \citep{mckay1981practical,aflalo2015convex},
%graph clustering \citep{titouan2019optimal,xu2020gromov},
%graph classification \citep{titouan2019optimal,vincent2021online},
%graph generation \citep{xu2020gromov},
%and network retrieval \citep{berretti2001efficient,ozer2002graph}.
%It also has applications to many problems of industrial or academic interest, such as
%linking user accounts in social platforms \citep{shu2017user,wang2019user},
%entity alignment in knowledge graphs \citep{sun2020knowledge,pei2020rea},
%and matching keypoints across two images \citep{sarlin2020superglue,wang2020zero},
%to name a few.




==> sections/methodology.tex <==
Motivated by our perspective, we propose a new graph matching algorithm \method{}.
Crucial details are discussed in this section.
%We present the proposed \method{} in Algorithm \ref{alg:method} and discuss about some crucial details in this section.




\subsection{Objective Function}


Assuming $|\VM^\src|\le|\VM^\tar|$, graph matching aims to find an injective mapping $\pi:\VM^\src\to\VM^\tar$ that matches nodes in $\GM^\src$ to nodes in $\GM^\tar$.
$\pi$ is also commonly represented as a matching matrix $\TB=\{0,1\}^{|\VM^\src|\times |\VM^\tar|}$,
where $T_{ii'}=1$ if node $i$ in $\GM^\src$ is matched to node $i'$ in $\GM^\tar$, and $T_{ii'}=0$ otherwise (eg. \citep{fey2019deep,heimann2021refining}).
%Assuming $\GM^\src$ has fewer or equal number of nodes than $\GM^\tar$ without loss of generality $|\VM^\src|\le|\VM^\tar|$, 
We find the matching matrix by solving the following quadratic assignment problem
\begin{equation}\label{eq:discrete formulation}
	\min_{\TB\in\PM^f}\sum_{i=1}^{|\VM^\src|}\sum_{j=1}^{|\VM^\src|}\sum_{i'=1}^{|\VM^\tar|}\sum_{j'=1}^{|\VM^\tar|}d_{ii'jj'}T_{ii'}T_{jj'},
\end{equation}
where $d_{ii'jj'}$ is the cost for the pairwise assignment $(i,j)\rightarrow (i',j')$,
and the feasible domain is
\begin{equation*}
	\PM^f=\Big\{\TB\in\{0,1\}^{|\VM^\src|\times |\VM^\tar|}\Big|\TB\oneB=\oneB,\TB^\top\oneB\le\oneB\Big\},
\end{equation*}
where $\oneB$ is an all-ones vector.

Compared to \citep{xu2019gromov,xu2019scalable} that only use edge weights to define the alignment costs,
the cost $d_{ii'jj'}$ of \method{} exploits the local topological structure.
The $K$-th order heat diffusion wavelet allows us to define a new matrix $\BB^z=[B_{ij}^z]$ describing node dissimilarities within each graph, i.e.,
\begin{equation}
	B_{ij}^z=\begin{cases}
		&\bar{\Psi}-\Psi_{ij}^z,\text{ if }i\neq j,\\
		&0, \text{ else,}
	\end{cases}
\end{equation}
where $\Psi_{ij}^z$ is defined as Eq. (\ref{eq:heat diffusion wavelet}), $z=\src,\tar$ and constant $\bar{\Psi}>\max_{i,j,z}\Psi_{ij}^z$.
%Obviously, $B_{ij}^z=\bar{\Psi}$ if node $j$ is more than $K$ hops away from node $i$ and $\BB^z$ measures the local topology of each node.
The alignment cost incorporating the local topological structure is thus defined as $d_{ii'jj'}=(B_{ij}^\src-B_{i'j'}^\tar)^2$.

%Such formulation matches every node in $\GM^\src$ to a node in $\GM^\tar$ and hence is referred to as \emph{full matching} \citep{kazemi2015can}.
%In real-world applications, $\GM^\src$ and $\GM^\tar$ are often two partially overlapping subgraphs of an underlying supergraph, that is, some nodes in one graph may not
%exist in the other one.
%Thus, our method also considers \emph{partial matching} by replacing the constraint $\PM^f$ with $\PM^p$ given by
%\begin{equation*}
%	\PM^p=\Big\{\TB\in\{0,1\}^{|\VM^\src|\times |\VM^\tar|}\Big|\TB\oneB\le\oneB,\TB^\top\oneB\le\oneB, \oneB^\top\TB\oneB=b\Big\},
%\end{equation*}
%where $b\le\min\{|\VM^\src|,|\VM^\tar|\}$.
%When the equality holds, partial matching is reduced to full matching.

\subsection{Optimization}\label{sec:optimization}
By relaxing $\TB\in\{0,1\}^{|\VM^\src|\times |\VM^\tar|}$ to $\TB\in[0,1]^{|\VM^\src|\times |\VM^\tar|}$,
Problem (\ref{eq:discrete formulation}) is converted to solving the partial GW discrepancy
\begin{equation}\label{eq:continuous formulation}
	\min_{\TB\in\Pi^{|\VM^\src|}}\ell(\TB):=\sum_{i=1}^{|\VM^\src|}\sum_{j=1}^{|\VM^\src|}\sum_{i'=1}^{|\VM^\tar|}\sum_{j'=1}^{|\VM^\tar|}d_{ii'jj'}T_{ii'}T_{jj'},
\end{equation}
where $\Pi^{|\VM^\src|}=\{\TB\in[0,1]^{|\VM^\src|\times |\VM^\tar|}\Big|\TB\oneB=\oneB,\TB^\top\oneB\le\oneB, \oneB^\top\TB\oneB=|\VM^\src|\}$,
since we assume $|\VM^\src|\le|\VM^\tar|$.

The most common algorithm for solving Problem (\ref{eq:continuous formulation}) is gradient descent that iteratively updates $\TB$ as follows
\begin{equation}\label{eq:gd}
	\TB^{(\tau+1)}=\proj_{\Pi^{|\VM^\src|}}\Big\{\TB^{(\tau)}-\eta^{(\tau)}\nabla \ell(\TB^{(\tau)})\Big\}.
\end{equation}

Mirror descent takes into account the geometry of the feasible domain \citep{bubeck2015convex}, and is better-suited to Problem (\ref{eq:continuous formulation}).
Mirror descent is given by the recurrence
\begin{equation}\label{eq:md 0}
	\TB^{(\tau+1)}=\argmin_{\TB\in\Pi^{|\VM^\src|}}\langle \nabla \ell(\TB^{(\tau)}),\TB\rangle+\frac{1}{\eta^{(\tau)}}D_\psi(\TB,\TB^{(\tau)}),
\end{equation}
where $D_\psi(\TB,\TB^{(\tau)})$ stands for the Bregman divergence.
%where $D_\psi(\TB,\TB^{(\tau)})=\psi(\TB)-\psi(\TB^{(\tau)})-\langle\nabla\psi(\TB^{(\tau)}),\TB-\TB^{(\tau)}\rangle$ stands for the Bregman divergence generated by a strongly convex and continuously differentiable function $\psi(\TB)$.
When one selects KL-divergence as the Bregman divergence,
(\ref{eq:md 0}) becomes
\begin{equation}\label{eq:md}
	\TB^{(\tau+1)}=\proj_{\Pi^{|\VM^\src|}}\Big\{\TB^{(\tau)}\odot\exp\big(-\JB-\eta^{(\tau)}\nabla\ell(\TB^{(\tau)})\big)\Big\},
\end{equation}
where $\JB$ is the all-ones matrix, $\odot$ is the element-wise multiplication, and the exponentiation is also element-wise.
%Adopting the aforementioned assignment costs, the gradient has the following form,
%\begin{equation}\label{eq:gradient}
%	\nabla\ell(\TB)=h(\BB^\src)\oneB\otimes\pB+\oneB\otimes h(\BB^\tar)\qB-2\BB^\src\TB^{(\tau)}\BB^\tar
%\end{equation}
%where $\pB=\TB\oneB$, $\qB=\TB^\top\oneB$, $h$ denotes the element-wise square and $\otimes$ is the outer product of two vectors \citep{peyre2016gromov}.

If the projections in Eq. (\ref{eq:gd}) and (\ref{eq:md}) are based on the KL-divergence, they can be solved via periodic projections \citep{benamou2015iterative}.
\method{} converges to an $\epsilon$-stationary point with the number of mirror descent iterations $\OM(\frac{1}{\epsilon^2})$,
by Corollary 3.1 of \citet{zhang2018convergence}.
%Let $\CM_1=\{\TB|\TB\oneB\le\oneB\}$, $\CM_2=\{\TB|\TB^\top\oneB\le\oneB\}$, and $\CM_3=\{\TB|\oneB^\top\TB\oneB=|\VM^\src|\}$.
%The KL-divergence based projection onto these three sets have closed forms
%\begin{equation}\label{eq:periodic projections}
%	\begin{aligned}
%		\proj_{\CM_1}^\KL(\TB)&=\Diag\Big(\min\{\frac{\oneB}{\TB\oneB},\oneB\}\Big)\TB,\\
%		\proj_{\CM_2}^\KL(\TB)&=\Diag\Big(\min\{\frac{\oneB}{\TB^\top\oneB},\oneB\}\Big)\TB,\\
%		\proj_{\CM_3}^\KL(\TB)&=\TB\frac{|\VM^\src|}{\oneB^\top\TB\oneB},
%	\end{aligned}
%\end{equation}
%where the division and minimum is element-wise.
%Extending the indexing of the sets by $3$-periodicity so that they satisfy $\CM_{k+3}=\CM_k$ for all $k\in\NBB$, one computes $\forall k>0$, $\TB^{(k,\tau)}=\proj_{\CM_k}^\KL(\TB^{(k-1,\tau)})$ with $\TB^{(0,\tau)}=\TB^{(\tau)}\odot\exp\big(-\JB-\eta^{(\tau)}\nabla\ell(\TB^{(\tau)})\big)$.
%%%%%%%%%%%%%%%  new description  %%%%%%%%%%%%%%%%%%%%%%
%A periodic sequence $\{\CM_k|k>0 \text{ and }k\in\NBB\}$ is constructed so that they satisfy $\CM_{k+3}=\CM_k$ for all positive integers $k$,
%where $\CM_1=\{\TB|\TB\oneB\le\oneB\}$, $\CM_2=\{\TB|\TB^\top\oneB\le\oneB\}$, and $\CM_3=\{\TB|\oneB^\top\TB\oneB=|\VM^\src|\}$.
%For all $k>0$, one computes $\TB^{(k,\tau)}=\proj_{\CM_k}^\KL(\TB^{(k-1,\tau)})$ with $\TB^{(0,\tau)}=\TB^{(\tau)}\odot\exp\big(-\JB-\eta^{(\tau)}\nabla\ell(\TB^{(\tau)})\big)$.
%The KL-divergence based projection onto these three sets have closed forms
%\begin{equation}\label{eq:periodic projections}
%	\begin{aligned}
%		\proj_{\CM_1}^\KL(\TB)&=\Diag\Big(\min\{\frac{\oneB}{\TB\oneB},\oneB\}\Big)\TB,\\
%		\proj_{\CM_2}^\KL(\TB)&=\TB\Diag\Big(\min\{\frac{\oneB}{\TB^\top\oneB},\oneB\}\Big),\\
%		\proj_{\CM_3}^\KL(\TB)&=\TB\frac{|\VM^\src|}{\oneB^\top\TB\oneB},
%	\end{aligned}
%\end{equation}
%where the division and minimum is element-wise.
%The following proposition states the convergence of periodic projections.
%\begin{proposition}[Proposition 5 of \citet{benamou2015iterative}]
%	$\TB^{(k,\tau)}$ converges towards the unique projection $\argmin_{\TB\in\PM^p}\KL(\TB\|\TB^{(0,\tau)})$.
%\end{proposition}

%\method{} updates the transport plan as (\ref{eq:md}).
%The convergence is guaranteed as follows and the proof is given in the appendix.
%\begin{proposition}[Corollary 3.1 of \citet{zhang2018convergence}]\label{prop:md}
%	\method{} converges to an $\epsilon$-stationary point with the number of mirror descent iterations $\OM(\frac{1}{\epsilon^2})$.
%\end{proposition}

\paragraph{Computational complexity.}
The complexity for calculaing the heat diffusion wavlets is $\OM(KV^3)$ where $V=\max\{|\VM^\src|,|\VM^\tar|\}$.
Due to the two matrix multiplication steps of the term $\BB^\src\TB\BB^\tar$,
calculating the gradient involves computational complexity $\OM(V^3)$.
Note that the matrix multiplication is highly parallelizable and well-suited to modern computing architectures like GPUs.
$\OM(V^2)$ cost is induced by periodic projections.
Therefore, if we run projected mirror descent for $N$ iterations, each of which has $T$ periodic projections,
$\OM\big(NTV^2+(N+K)V^3\big)$ computational cost is required in learning the optimal transport.
Such complexity is of the same order as state-of-the-art methods like \citet{xu2019gromov,konar2020graph,scott2021graph,heimann2021refining},
and lower than \citet{neyshabur2013netal,malod2015graal,fan2020spectral}.
Considering the sparsity of edges in \realworld{} graphs,
the complexity can be reduced to $\OM\big(NTV^2+(N+K)VE\big)$ where $E=\max\{|\EM^\src|,|\EM^\tar|\}$.

%To further reduce the computational complexity and memory footprint,
%we can recursively partition graphs into aligned sub-graph pairs,
%across which the node correspondence can be found by \method{} (just as techniques proposed in \citep{xu2019scalable}).
%The time and memory complexity are reduced to $\OM\big(N(E+V)\log V+NTV^2\big)$ and $\OM(E+V)$, where $E=\max\{|\EM^\src|,|\EM^\tar|\}$.
%Note that directly partitioning graphs like \citet{xu2019scalable} modifies the local topology of many nodes and thus hurts the alignment accuracy.
%By precomputing and storing the local topological information in $\BB^z$, such problem is overcome.




\begin{algorithm}[ht]
	\caption{\method{} \label{alg:method}}
	\begin{algorithmic}[1]
		\State {\textbf{Input:}} Total rounds $T$, graphs $\GM^\src$ and $\GM^\tar$, initial transport plan $\TB^{(0)}$.
		\State {\textbf{Output:}} Correspondence set $\CM$.
		\State Calculate and store matrices $\BB^\src$ and $\BB^\tar$.
		\For{$\tau=0,\dots,T-1$}
		\State Update $\TB^{(\tau+1)}$ by iteration \ref{eq:md}.
		\EndFor
		\State $\tilde{\TB}=\TB^{(T)}$
		\State Initialize correspondence set $\CM=\emptyset$
		\For{$i\in\VM^\src$}
		\State $i'=\arg\max_{i'} \tilde{T}_{ii'}$.
		\State $\CM=\CM\cup\{(i,i')\}$
		\EndFor
	\end{algorithmic}
\end{algorithm}

\method{} is summarized in Algorithm \ref{alg:method}.
The matching cost is based on heat diffusion wavelets.
It updates the transport plan using mirror descent.
By choosing the largest $\tilde{T}_{ii'}$ for each i, we find the correspondence.

%\begin{algorithm}[ht]
%	\caption{\method{} \label{alg:method}}
%	\begin{algorithmic}[1]
%		\State {\textbf{Input:}} Total rounds $T$, graphs $\GM^\src$ and $\GM^\tar$, matrices $\BB^\src$ and $\BB^\tar$, and total transport mass $b$.
%		\State {\textbf{Output:}} Correspondence set $\CM$.
%		\State Randomly initialize $\TB_0\in\PM^p$.\Comment{If $b<|\VM^\src|$, \method{} conducts partial matching.}
%		%		\State Calculate and store heat diffusion wavelets.
%		\For{$\tau=0,\dots,T-1$}
%		\State Update $\TB_{\tau+1}$ by iteration \ref{eq:mirror descent}.
%		\EndFor
%		\State $\tilde{\TB}=[\TB_T,\oneB-\TB_T\oneB]$\Comment{The extended transport plan $\tilde{\TB}\in\RBB^{|\VM^\src|\times(|\VM^\tar|+1)}$.}
%		\State Initialize correspondence set $\CM=\emptyset$
%		\For{$i\in\VM^\src$}
%		\State $i'=\arg\max_{i'} \tilde{T}_{ii'}$.
%		\If{$i'\neq(|\VM^\tar|+1)$}\Comment{Otherwise, $i$ is matched to the dummy point.}
%		\State $\CM=\CM\cup\{(i,i')\}$
%		\EndIf
%		\EndFor
%	\end{algorithmic}
%\end{algorithm}
%
%\method{} is summarized in Algorithm \ref{alg:method}.
%We use the learned $\TB_T$ to construct an extended transport plan $\tilde{\TB}=[\TB_T,\oneB-\TB_T\oneB]\in\RBB^{|\VM^\src|\times(|\VM^\tar|+1)}$.
%This can be thought of adding a \emph{dummy} point to $\GM^\tar$, which is similar to \citep{chapel2020partial}.
%By choosing the largest $\tilde{T}_{ii'}$ for each i, we find the correspondence.

\subsection{Topological interpretation}\label{sec:interpretation}
%The key principle for matching undirected and unattributed graphs is the topological consistency:
%nodes that are close in one graph should be matched to nodes that are close in the other graph \citep{heimann2021refining}.
%\method{} achieves the topological consistency by using assignment costs that quantify the local topological consistency,
%which we formulate in this subsection.

Adopting the aforementioned assignment costs, the gradient has the following form,
\begin{equation}\label{eq:gradient}
	\nabla\ell(\TB)=h(\BB^\src)\oneB\otimes\pB+\oneB\otimes h(\BB^\tar)\qB-2\BB^\src\TB^{(\tau)}\BB^\tar
\end{equation}
where $\pB=\TB\oneB$, $\qB=\TB^\top\oneB$, $h$ denotes the element-wise square and $\otimes$ is the outer product of two vectors \citep{peyre2016gromov}.
Substituting Eq. (\ref{eq:gradient}) into the mirror descent update \ref{eq:md},  Eq. (\ref{eq:md}) can be rewritten as
\begin{equation}\label{eq:mirror descent}
	\TB^{(\tau+1)}=\proj_{\Pi^{|\VM^\src|}}\Big(\frac{1}{e}\TB^{(\tau)}\odot\SB(\TB)^{\eta(\tau)}\Big),
\end{equation}
where $\SB(\TB)=\exp\Big(2\BB^\src\TB\BB^\tar-h(\BB^\src)\pB\otimes\oneB-\oneB\otimes h(\BB^\tar)\qB\Big)$ and the exponentiation is element-wise.

When $K=1$, the topology violation has a more intuitive interpretation.
\begin{proposition}\label{prop:relationship with MNC}
	When one only uses one-hop neighborhood information (i.e., $K=1$) to match two graphs of the same number of nodes,
	\begin{equation*}
		\begin{aligned}
			\exp\big(-d(i,i';\TB)\big)=\frac{\exp\Big(t|\tilde{\NM}_1^\src(i;\pi)\cap\NM_1^\tar(i')|\Big)}{\exp\Big(t|\tilde{\NM}_1^\src(i;\pi)\cup\NM_1^\tar(i')|\Big)},
		\end{aligned}
	\end{equation*}
	where $\TB\in\PM^f$, $\tilde{\NM}_k^\src(i;\pi)=\{j'\in\VM^\tar|\exists j\in\NM_k^\src(i) \st \pi(j)=j'\}$, and the bijective is given by $\pi(i)=\argmax_{i'}T_{ii'}$.
	Compared to $\operatorname{MNC}(i, i';\pi)=\frac{\left|\tilde{\NM}_1^{\src}(i;\pi) \cap \NM_{1}^\tar(i')\right|}{\left|\tilde{\NM}_1^{\src}(i;\pi) \cup \NM_{1}^\tar(i')\right|}$ \citep{chen2020cone,heimann2021refining},
	$\exp\big(-d(i,i';\TB)\big)\le\MNC(i,i';\pi)$ when $t=1$ and $\tilde{\NM}_1^{\src}(i;\pi) \cap \NM_{1}^\tar(i')$ is not empty.
\end{proposition}


%The transport distance between the heat diffusion wavelet coefficients,
%$d(i,i';\TB)=\sum_{j=1}^{|\VM^\src|}\sum_{j'=1}^{|\VM^\tar|}T_{jj'}(B_{ij}^\src-B_{i'j'}^\tar)^2$,
%measures the topology violation between nodes $i$ and $i'$ for matching matrix $\TB$.
%Based upon $d(i,i';\TB)$, we can define the \emph{\Quantity} (\Quan{}) that measures the topological consistency of node $i$ and node $i'$ given matching matrix $\TB$ as\footnote{Defining similarity values based on distance functions is common in machine learning literature. For example, in \citet{hinton2002stochastic,van2008visualizing}, the similarity value between two embedding vectors $\zB_i$ and $\zB_j$ with distance $d(\zB_i,\zB_j)$ is defined as $\exp\big(-d(\zB_i,\zB_j)\big)$.}
%\begin{equation}
%	\maQuan(i,i';\TB)=e^{-d(i,i';\TB)}.
%\end{equation}

%Eq. (\ref{eq:mirror descent}) implies that each iteration (\ref{eq:md}) increases alignment scores for node pairs that have high \Quan{}.
%Indeed, the \Quan{} for all node pairs $(i, i')$ given the alignment matrix $\TB$, can be written as a matrix $\SB=[S_{ii'}]$ 
%	\begin{equation*}
%		\SB(\TB)=\exp\Big(2\BB^\src\TB\BB^\tar-h(\BB^\src)\pB\otimes\oneB-\oneB\otimes h(\BB^\tar)\qB\Big),
%	\end{equation*}
%such that $\ehdc(i,i';\TB)=S_{ii'}$.
%Therefore, iteration $\tau$ can also be written as $\TB^{(\tau+1)}=\proj_{\Pi^{|\VM^\src|}}\Big(\TB^{(\tau)}\odot\exp(-\JB)\odot\SB(\TB^{(\tau)})^{\eta^{(\tau)}}\Big)$, where the exponentiation is element-wise.

%Eq. (\ref{eq:mirror descent}) implies that each iteration (\ref{eq:md}) increases alignment scores for node pairs that have high \Quan{}.
%Indeed, we have the following proposition.
%\begin{proposition}\label{prop:matrix Quan}
%	The \Quan{} for all node pairs $(i, i')$ given the alignment matrix $\TB$, can be written as a matrix $\SB=[S_{ii'}]$ 
%	\begin{equation*}
%		\SB(\TB)=\exp\Big(2\BB^\src\TB\BB^\tar-h(\BB^\src)\pB\otimes\oneB-\oneB\otimes h(\BB^\tar)\qB\Big),
%	\end{equation*}
%	such that $\ehdc(i,i';\TB)=S_{ii'}$.
%\end{proposition}
%Therefore, iteration $\tau$ can also be written as $\TB^{(\tau+1)}=\proj_{\Pi^{|\VM^\src|}}\Big(\TB^{(\tau)}\odot\exp(-\JB)\odot\SB(\TB^{(\tau)})^{\eta^{(\tau)}}\Big)$, where the exponentiation is element-wise.

We demonstrate that low topology violation for matched node pairs is a necessary condition for accurate alignment.
%On the one hand, accurate alignment entails high \Quan{}.
In particular, if $\GM^\src$ is isomorphic to a subgraph of $\GM^\tar$ that is induced by the true counterpart nodes,
up to a few noisy or missing edges,
$d\big(i,\pi^*(i);\TB^*\big)$ values are low where $\pi^*:\VM^\src\to\VM^\tar$ and $\TB^*=[T_{ii'}^*]$ are the true matching and its matrix form, respectively.
This is formalized in the following theorem.
\begin{theorem}\label{thm:principle}
	Let $\DeltaB^{(k)}=[\Delta^{(k)}_{jj'}]\in\RBB^{|\VM^\src|\times|\VM^\tar|}$ denote the perturbation to the edge structure, which is given by $\DeltaB^{(k)}=(\LB^\src)^k-\TB^{*}(\LB^\tar)^k\TB^{*\top}$.
	Assume that for all $i$,
	the perturbation to the local topology is bounded by $\sum_{j\in\NM_k^\src(i),j'\in\NM_k^\tar(\pi^*(i'))}|\Delta^{(k)}_{jj'}|^2\le\epsilon^{(k)}$.
	Then $\maQuan\big(i,\pi^*(i);\TB^*\big)$ can be bounded from below as follows:
	\begin{equation*}
		d\big(i,\pi^*(i);\TB^*\big)\le K\sum_{k=1}^{K}\Big(\frac{(-t)^k}{k!}\Big)^2\epsilon^{(k)}.
	\end{equation*}
%	\begin{equation*}
%		\maQuan\big(i,\pi^*(i);\TB^*\big)\ge\exp\Big(-K\sum_{k=1}^{K}\Big(\frac{(-t)^k}{k!}\Big)^2\epsilon^{(k)}\Big).
%	\end{equation*}
\end{theorem}
%Theorem \ref{thm:principle} implies that $\maQuan\big(i,\pi^*(i);\TB^*\big)$ is close to $1$ for a small $s$.
%When $k$ is small, $\epsilon^{(k)}$ is small.
%As is required by heat diffusion wavelet, $s$ is usually small.
%Therefore, by choosing a small $s$, $\maQuan\big(i,\pi^*(i);\TB^*\big)$ is close to $1$.
The small-world property of real graphs suggests that a small $K$ is enough in practice \citep{watts1998collective}.
To capture local topology, $t$ is a small value \citep{tsitsulin2018netlsd,donnat2018learning}.
Therefore, $d\big(i,\pi^*(i);\TB^*\big)$ is close to 0.
%Therefore, $\maQuan\big(i,\pi^*(i);\TB^*\big)$ is close to $1$.

The mirror descent-based update allows $d\big(i,\pi^*(i);\TB^*\big)$ values for matched node pairs to decrease gradually,
which we formalize in the following theorem.
%The high-level idea is that when the topology violation for true node pairs is much lower than the topology violation
\begin{theorem}\label{thm:mirror descent assumptions}
	When we use \method{} to match graphs of the same number of nodes,
	if the following assumptions hold:
	\begin{enumerate}
		\item $\alpha^{(\tau)}\ge d(i,\hat{i};\TB^{(\tau)})$ for all $i$ where $\hat{i}=\argmax_{i'}T_{ii'}$,
		\item $\beta^{(\tau)}\le d(i,i';\TB^{(\tau)})$ for all $i$ where $i'\neq \hat{i}$,
		\item $|\VM^\src|\exp(\alpha^{(\tau)}\eta^{(\tau)})\le\exp(\beta^{(\tau)}\eta^{(\tau)})$ for all $i$,
	\end{enumerate}
	the topology violation values for all $(i,\hat{i})$ decrease at iteration $\tau$, $d(i,\hat{i};\TB^{(\tau+1)})\ge d(i,\hat{i};\TB^{(\tau)})$.
\end{theorem}
According to Proposition \ref{prop:relationship with MNC} and Theorem \ref{thm:mirror descent assumptions}, \method{} with $K=1$ and $t=1$ can also be viewed as maximizing a lower bound of $\operatorname{MNC}(i, i^*;\pi^*)$ for all true node pairs.


%We further note that the true matching matrix $\TB^*$ is a fixed point for the mirror descent-based optimization.
%\begin{theorem}\label{thm:fixed point}
%	$\TB^*$ is a fixed point for iteration (\ref{eq:md}).
%\end{theorem}


%To alleviate (near) structural indistinguishability,
%one may take a larger neighborhood into account.

%On the other hand, misalignment may occur but only for structurally indistinguishable nodes, as is shown in Theorem \ref{thm:indistinguishable}.
%
%\begin{theorem}\label{thm:indistinguishable}
%	If $\GM^\src$ is isomorphic to a subgraph of $\GM^\tar$, suppose that there exists $\pi(\cdot)$ that yields $\maQuan=1$ for all matched node pairs.
%	Then, if $\pi$ misaligns a node $i$ to a node $i'$ instead of the true counterpart $i^*$,
%	it is because $\NM_k^\tar(i')$ is isomorphic to $\NM_k^\tar(i^*)$.
%\end{theorem}

%When $K=1$, \Quan{} has a more intuitive interpretation, which needs the following definition.
%\begin{definition}[mapped neighborhood]
%	The mapped neighborhood of node $i\in\VM^\src$ is the set of nodes in $\GM^\tar$ onto which $\pi$ maps $i$'s neighbors, i.e., $\tilde{\NM}_k^\src(i;\pi)=\{j'\in\VM^\tar|\exists j\in\NM_k^\src(i) \st \pi(j)=j'\}$.
%\end{definition}

%\citeauthor{chen2020cone} \citeyear{chen2020cone} and \citeauthor{heimann2021refining} \citeyear{heimann2021refining} define the \emph{matched neighborhood consistency} (MNC) of node $i$ in $\GM^\src$ and node $i'$ in $\GM^\tar$ to be the Jaccard similarity of the sets $\tilde{\NM}_1^{\src}(i;\pi)$ and $\NM_{1}^\tar(i')$, i.e., $\operatorname{MNC}(i, i';\pi)=\frac{\left|\tilde{\NM}_1^{\src}(i;\pi) \cap \NM_{1}^\tar(i')\right|}{\left|\tilde{\NM}_1^{\src}(i;\pi) \cup \NM_{1}^\tar(i')\right|}$.
%When $K=1$ and two graphs of the same number of nodes are to be matched, \Quan{} can be reduced to a form similar to MNC, which is stated in the following proposition.



%We further reveal that RefiNA proposed by \citeauthor{heimann2021refining}\citeyear{heimann2021refining} essentially maximizes the edge correctness (EC),
%which is defined as the ratio of the number of edges conserved by $\pi$ to the
%number of edges in the source network
%\citep{patro2012global},
%%\citep{patro2012global,saraph2014magna,sun2015simultaneous,mamano2017sana,xu2019scalable},
%\begin{equation*}
%	\maEC(\pi)=\frac{|\pi(\EM^\src)|}{|\EM^\src|}, \where \pi(\EM^\src)=\{\big(\pi(i),\pi(j)\big)\in\EM^\tar|\forall (i,j)\in\EM^\src\}.
%\end{equation*}
%RefiNA iteratively increases alignment scores for nodes that have high relaxed numerator values of MNC.
%Representing $\pi$ with the matrix form $\TB$ and relaxing the binary matching matrix to $\PM^f$,
%the gradient of $\maEC$ with respect to $\TB$ is $\WB^\src\TB\WB^\tar$, the relaxed numerator values of MNC values \citep{heimann2021refining}.
%As is shown in \citet{saraph2014magna}, EC does not penalize alignments mapping sparser network regions to denser ones, which negatively affects the alignment accuracy and leaves room for improvement.


















==> sections/topology.tex <==
%We present our topological view for OT-based graph matching methods by three steps:
%1) Each entry of the gradient with respect to the transport plan can be viewed as the topology violation of the corresponding node pair and existing OT-based graph matching methods increase the alignment scores of node pairs with low violation values.
%2) Under suitable assumptions,
%such procedure can reduce the topology violation of matched node pairs.
%%and increase the probability that true node pairs are matched.
%3) Low topology violation of all matched node pairs is a necessary condition for accurate matching.

We present our topological view for OT-based graph matching methods by three steps:
1) Each entry of the gradient with respect to the transport plan, denoted as $G_{ii'}(\TB)$, can be viewed as the topology violation of node pair $(i,i')$;
2) Because of the feasible domain, gradient-based methods increase $T_{ii'}$ if $G_{ii'}(\TB)$ is large and decrease $T_{ii'}$ if $G_{ii'}(\TB)$ is small,
so that overall topology violation is reduced;
3) Under suitable assumptions,
the topology violation values of matched node pairs, denoted as $G_{i\hat{i}}$'s where node $i$ is matched to node $\hat{i}$, tend to $0$,
which is a sufficient and necessary condition for matching structurally distinguishable nodes.

\subsection{Topology Violation and OT}

OT-based methods adjust the transport plan dynamically according to the topology violation.
%Following the definition of \emph{measure networks} \citep{chowdhury2019gromov,xu2019gromov},
Mainstream methods assign two distributions $\muB^\src=[\mu^\src_i]$ and $\muB^\tar=[\mu^\tar_i]$ to the source graph $\GM^\src=(\VM^\src,\EM^\src,\WB^\src)$ and the target graph $\GM^\tar=(\VM^\tar,\EM^\tar,\WB^\tar)$ respectively \citep{xu2019gromov,xu2019scalable,chowdhury2019gromov,titouan2019optimal,barbe2020graph},
where
\begin{equation*}
	\mu^z_i=\frac{\sum_{j=1}^{|\VM^z|} W_{ij}^z}{\sum_{i=1}^{|\VM^z|}\sum_{j=1}^{|\VM^z|}W_{ij}^z}, \text{ for }z=\src,\tar.
\end{equation*}
%Without loss of generality, we assume $|\VM^\src|\le|\VM^\tar|$.
A cost matrix $\CB^z=[C_{ij}^z]\in\RBB^{|\VM^z|\times|\VM^z|}$ is further defined with each $C_{ij}^z$ characterizing the dissimilarity between vertices $i$ and $j$.
%for example,
%$C_{ij}^z=\frac{1}{1+W_{ij}^z}$ \citep{xu2019gromov}.%例子都写出来，别管全局和局部
The GW distance between $\GM^\src$ and $\GM^\tar$ is then defined as
\begin{equation}\label{eq:Xu GW}
		GW(\muB^\src,\muB^\tar)=\min_{\TB\in\Pi(\muB^\src,\muB^\tar)}\sum_{i=1}^{|\VM^\src|}\sum_{j=1}^{|\VM^\src|}\sum_{i'=1}^{|\VM^\tar|}\sum_{j'=1}^{|\VM^\tar|}(C_{ij}^\src-C_{i'j'}^\tar)^2T_{ii'}T_{jj'}.
\end{equation}
%The transport plan $\TB^*$ that attains the minimum indicates the node correpsondence across the two graphs.
Node $i\in\VM^\src$ is matched to $\hat{i}\in\VM^\tar$ where $\hat{i}=\argmax_{i'}T^*_{ii'}$ and $\TB^*=[T^*_{ii'}]$ attains the minimum of Eq. (\ref{eq:Xu GW}).

Existing methods update the transport plan using the gradient that arises from Problem (\ref{eq:Xu GW}) \citep{xu2019gromov,xu2019scalable,titouan2019optimal,barbe2020graph} and the gradient has the following form:
\begin{equation}
	\GB(\TB)=h(\CB^\src)\oneB\otimes\oneB+\oneB\otimes h(\CB^\tar)\oneB-2\CB^\src\TB\CB^\tar,
\end{equation}
where $h$ denotes the element-wise square and $\otimes$ is the outer product of two vectors \citep{peyre2016gromov}.

The gradient with respect to the transport plan $\GB(\TB)=[G_{ii'}(\TB)]$ admits topological interpretation.
In particular, each entry can be written as the transport distance,
%between two discrete measures induced by nodes $i$ and $i'$ respectively,
\begin{equation*}\label{eq:gradient interpretation}
	G_{ii'}(\TB)=\sum_{j=1}^{|\VM^\tar|}\sum_{j'=1}^{|\VM^\tar|}T_{jj'}(C_{ij}^\src-C_{i'j'}^\tar)^2,%局部还是全局？和C取值有关系
\end{equation*}
and can be interpreted as the \emph{violation} of the local topology of node $i\in\VM^\src$ and $i'\in\VM^\tar$ given the current transport plan $\TB$.
%Exising methods gradually improve the matching accuracy by 
Since the transport plan satisfies the constraints $\TB\in\Pi(\muB^\src,\muB^\tar)$,
existing methods increase $T_{jj'}$ with small $G_{ii'}(\TB)$ in each iteration to reach a matching consensus in local neighborhoods between graphs.
This is essentially in the same spirit as \citeauthor{fey2019deep} \citeyear{fey2019deep}'s work,
which matches attributed graphs in a supervised manner.

\subsection{Reducing Topology Violation}

%Increasing the alignment score $T_{ii^*}$ where node $i^*$ is the true counterpart of node $i$, can in turn reduce the transport distance $G_{ii^*}(\TB)$, i.e., improve the topology conservation of $(i,i^*)$.
%This also increases the possibility that $i^*$ is matched to $i$. 
%Denote 
%Increasing the alignment score of true node pairs can in turn reduce the transport distance $G_{ii^*}(\TB)$.
%\begin{proposition}\label{prop:each step}
%	Denote the recurrence by $\TB^{(\tau+1)}=\iota\big(\TB^{(\tau)}\big)$.
%	For isomorphic graphs,
%	the transport distances of true node pairs decrease at iteration $\tau$, $G_{ii^*}(\TB^{(\tau+1)})\le G_{ii^*}(\TB^{(\tau)})$,
%	if $T_{ii'}^{(\tau+1)}\le T_{ii'}^{(\tau)}$ for all $i$ and $i'\neq i^*$.
%\end{proposition}


Increasing the alignment score $T_{ii'}$ if the topology violation $G_{ii'}(\TB)$ is small,
can in turn reduce the topology violation of matched node pairs,
when matched node pairs have similar local topology.
We first formalize the concept of local neighborhoods.
\begin{definition}[$k$-hop neighborhood]
	The $k$-hop neighborhood of node $i$ in graph $z$, denoted by $\NM_k^z(i)$, is the subgraph of $\GM^z$ induced by all nodes that are $k$ or fewer hops away from node $i$, where $z=\src,\tar$.
\end{definition}


\begin{proposition}\label{prop:each step}
	Denote the recurrence by $\TB^{(\tau+1)}=\iota\big(\TB^{(\tau)}\big)$.
	When the following assumptions hold:
	\begin{enumerate}
		\item $\GM^\src$ and $\GM^\tar$ are isomorphic,
		\item for all $i\in\VM^\src$, $\NM_k^\src(i)$ is isomorphic to $\NM_k^\tar(\hat{i})$ where $\hat{i}$ is the matched node for $i$, $\hat{i}=\argmax_{i'}T_{ii'}$,
		\item the cost matrix quantifies the local topology, i.e., if node j is more than $k$ hops away from node $i$, $C_{ij}^z=\bar{\Psi}$ is large for $z=\src,\tar$,
		\item $T_{ii'}^{(\tau+1)}\le T_{ii'}^{(\tau)}$ for all $i$ and $i'\neq \hat{i}$,
	\end{enumerate}
	the transport distances of all matched node pairs decrease at iteration $\tau$, $G_{i\hat{i}}(\TB^{(\tau+1)})\le G_{i\hat{i}}(\TB^{(\tau)})$.%会不会降到大于0的一个数就停下来了
\end{proposition}

In Sec. \ref{sec:method},
we propose a mirror descent-based method that match graphs by reducing topology violation.

%\subsection{Necessity of Small Topology Violation}
Low transport distance for all matched node pairs is a necessary condition for accurate alignment.

On the one hand, accurate matching entails low transport distance for matched node pairs.
For all true node pairs $(i,i^*)$ and the optimal transport plan $\TB^*=\argmin_{\TB\in\Pi(\muB^\src,\muB^\tar)}\sum_{ii'jj'}(C_{ij}^\src-C_{i'j'}^\tar)^2T_{ii'}T_{jj'}$, the transport distance is small, which is stated in the following proposition.
\begin{proposition}\label{prop:transport distance}
	For isomorphic graphs and $C_{ij}^z=\frac{1}{1+W_{ij}^z}$,%C不止可以取这种形式
%	denote the true matching matrix by $\TB^*$,
	the transport distance of all matched node pairs $(i,i^*)$ where $i^*=\argmax_{i'}T^*_{ii'}$ is 0,
	\begin{equation*}
		G_{ii^*}(\TB^*)=0,
	\end{equation*}
	while for node $i'\neq i^*$, the transport distance is generally large
	\begin{equation*}
		G_{ii'}(\TB^*)=\sum_{j=1}^{|\VM^\src|}\mu_j^\src(C_{ij}^\src-C_{i'j^*}^\tar)^2,
	\end{equation*}
	where $j^*=\argmax_{j'}T^*_{jj'}$.
\end{proposition}
Therefore, we aim to estimate the node correspondence by minimizing the transport distance for matched node pairs in this paper.

On the other hand, misalignment may still occur even if the transport distances for all matched node pairs are low.
This is due to (near) structural indistinguishability.
To illustrate this, consider an extreme case of matching two star graphs, each consisting of one center node connected to $n-1$ peripheral nodes \citep{heimann2021refining}.
Matching peripheral nodes to each other in any order leads to zero transport distances,
whatever the true correspondence of the peripheral nodes is.
Distinguishing such nodes from pure graph topology is impossible.
%In many cases, however, one may alleviate (near) structural indistinguishability by taking a larger neighborhood into account.

